Pregnant Questions: The Importance of Pragmatic Awareness in Maternal Health Question Answering

Questions posed by information-seeking users often contain implicit false or potentially harmful assumptions. In a high-risk domain such as maternal and infant health, a question-answering system must recognize these pragmatic constraints and go beyond simply answering user questions, examining them in context to respond helpfully. To achieve this, we study assumptions and implications, or pragmatic inferences, made when mothers ask questions about pregnancy and infant care by collecting a dataset of 2,727 inferences from 500 questions across three diverse sources. We study how health experts naturally address these inferences when writing answers, and illustrate that informing existing QA pipelines with pragmatic inferences produces responses that are more complete, mitigating the propagation of harmful beliefs.

==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/sections/00-abstract.tex <==
Questions posed by information-seeking users often contain implicit false or potentially harmful assumptions.
In a high-risk domain such as maternal and infant health, a question-answering system must recognize these pragmatic constraints and go beyond simply answering user questions, examining them in context to respond helpfully.
To achieve this, we study assumptions and implications, or \textit{pragmatic inferences}, made when mothers ask questions about pregnancy and infant care by collecting a dataset of 2,727 inferences from 500 questions across three diverse sources.
We study how health experts naturally address these inferences when writing answers, and  illustrate that informing  existing \qa{} pipelines with pragmatic inferences produces responses that are more complete, mitigating the propagation of harmful beliefs.


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/sections/10-introduction.tex <==
\input{tables/annotation-examples}

Humans have varying information needs when they ask questions~\cite{taylor1962process}.
Sometimes these needs are easily inferred from the surface form, such as in factoid questions (e.g. \textit{``Who is the 44th president of the United States''}).
However, in a question such as ``\textit{Is there a good non-dairy baby milk I can supplement for my newborn?}'', addressing the underlying false assumption ``\textit{Newborns can safely drink non-dairy milk}'' \textbf{becomes part of satisfying the unexpressed information need}. 
Complete answers to these types of questions must not only address the surface question itself, but also ``question the question'', critically examining its \textit{pragmatic needs}.

These needs become magnified in sensitive domains, such as consumer health or the legal domain.
In these settings, addressing pragmatic needs of questions involves proactively addressing false assumptions or implications in questions to ensure that the asker does not continue holding inaccurate beliefs that they may act on.
For example, a complete answer to the question about non-dairy milk for newborns should address that while non-dairy milk is viable for older babies, newborns and infants need human breast milk or dairy-based formula because they offer complete nutrition.

Language models have been shown to exhibit sycophancy~\cite{sharma2023towards}, sometimes adjusting responses to align with a human user's view.
However, helpful \abr{qa} systems should not only \textit{challenge} false or subjective assumptions in questions~\cite{Kim2022QA2QA} by verifying them against a vetted corpus, but also infer the asker's intent to make sure that its answer satisfactorily addresses their deeper information needs~\cite{taylor1962process}, just as humans do\footnote{``Pregnant'' in our title also refers to its secondary definition, ``full of meaning'' (as in ``a pregnant pause'') alluding to the idea that questions are laden with implicit beliefs.}.
\begin{figure}[t!]
\centering
\includegraphics[scale=0.76]{figures/teaser_figure.pdf}
\caption{We ask public health experts to identify assumptions and implications from questions and find that incorporating them in a \abr{qa} pipeline produces a more complete answer.}
\label{fig:presup-example}
\end{figure}

We construct a dataset\footnote{\scriptsize\url{https://github.com/nehasrikn/pragmatic-inferences-qa}} of 2,727 assumptions and implications in 500 questions (\S\ref{sec:data}) collected from three diverse sources to study (1) how humans embed such assumptions and implications in questions, and (2) the extent to which they are \textit{naturally} addressed in answers written by public health experts.
We then ground assumptions and implications, two primary ways humans embed beliefs in questions, in existing linguistic theory of presuppositions and implicatures respectively (\S\ref{sec:background}).
We refer to presupposition and implicature collectively as \textit{pragmatic inference}.
While recent work has focused on the task of detecting and addressing false \textit{presuppositions} in open-domain \qa{}~\cite{Yu2022CREPEOQ}, we find that false beliefs of question askers are more likely to present as implicatures than presuppositions (\S\ref{sec:ask-and-answer}).
We experiment with \textit{inducing} pragmatic behavior in existing \qa{} pipelines with state-of-the-art retrieval and machine reading models (\S\ref{sec:improve-qa}).
On questions with at least one highly plausible false pragmatic inference, our expert annotators rated responses from our pragmatic \abr{qa} system as more helpful and informative. 

Thus, \qa{} systems of the future must proactively address assumptions and implications in questions as they are increasingly deployed in sensitive domains.


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/sections/20-data.tex <==
In contrast with factoid \qa{}, systems deployed in \textit{sensitive} domains such as consumer health must proactively mitigate harm.
In these settings, correcting false assumptions is \textit{not optional}: systems must provide contextual answers that balance \textit{information completeness} with brevity.

Access to high quality healthcare in the United States vastly differs across socioeconomic backgrounds~\cite{becker2003socioeconomic}.
Such users are often likely to turn to accessible internet resources and---as of late---general purpose chatbots~\cite{palanica2019physicians}.
This motivates us to focus on maternal and infant care, a challenging area of consumer health where patients are concerned with \textit{both} their own physical health as well as the health of their child.

\input{tables/dataset}

To effectively study and induce pragmatic behavior in \abr{qa} systems, the evaluation questions we choose must reflect real-world experiences and situations for which there may not be a straightforward answer explicitly addressed in a single web document. 
For example, answers to Natural Questions~\cite[\nq{}]{kwiatkowski-etal-2019-natural}---a popular open-domain question-answering dataset---can be found directly in short extracted text snippets from Wikipedia (Table~\ref{table:dataset-examples}). 
In contrast, effectively answering the subjective questions sourced from Reddit requires commonsense reasoning and domain knowledge while identifying the asker's intent.

We carefully construct a dataset of questions from three distributionally distinct sources: a domain-specific \abr{qa} system we design and deploy to pregnant and postpartum participants we recruit~\cite{mane2023practical}, Reddit, and \nq{}.
Then, we introduce an annotation scheme to elicit assumptions and implications from these questions, validate their plausibility, and finally collect supporting evidence to determine their veracity.
Our final dataset contains 2,727 assumptions from 500 evaluation questions (Table~\ref{tab:dataset-sizes}). 
We also include 150 development questions used to train annotators and develop our \abr{qa} systems.


\subsection{Gathering a Diverse Set of Maternal and Infant Health Questions}

\paragraph{Maternal Health \abr{qa} System.}
We source questions come from a maternal and infant health-specific question answering system that we build~\citep{mane2023practical}, henceforth referred to as \abr{rosie}.
Users ask questions pertaining to pregnancy or infant health and are instructed that the \abr{qa} system does not have any personalized knowledge of their individual medical history or pregnancy.

This system operates over a corpus of web documents we construct\footnote{Corpus available upon request. We use \citet{barbaresi-2021-trafilatura} to scrape 408,000 web documents which we split into passages of 100 tokens following \citet{karpukhin-etal-2020-dense}.} from trusted sources including United States governmental and hospital organizations on maternal and infant health, and spans salient topics such as pregnancy and postpartum symptoms, developmental milestones, and infant safety.
Our end-to-end \abr{qa} system, \abr{rosie}, uses a passage retriever and reranker to provide web passages as answers to study participants via a mobile application.
We randomly sample 200 anonymized questions asked to \abr{rosie} for our evaluation set and 50 questions for our development set.

\paragraph{Reddit.} While the questions asked to \abr{rosie} do reflect real-world experiences, they are asked \textit{to an automatic system} and thus tend to include less situational detail or implicit content.
We turn to Reddit\footnote{\texttt{\url{https://www.reddit.com/}}} to capture long-tail questions that are about the diverse set of unique situations a new or expecting parent goes through. 
Table~\ref{table:dataset-examples} highlights some distributional differences between questions from Reddit and other data sources. 
Our questions come from four popular subreddits about maternal and infant health: \texttt{r/BabyBumps}, \texttt{r/breastfeeding}, \texttt{r/NewParents}, \texttt{r/Mommit}, and \texttt{r/beyondthebump} from the \texttt{pushshift}\footnote{\url{https://github.com/Watchful1/PushshiftDumps}} dump.

We develop a series of heuristics as a recall-oriented first step to identify questions with false or subjective assumptions.
We begin by selecting questions where an upvoted comment shows assumption-correcting behavior or where a user invokes their medical expertise, identified by a select list of discourse markers (Appendix~\ref{appendix:reddit}).
Of these, we only retain posts beginning with a ``wh'' word, filtering a few hundred thousand posts down to 2,858 questions. 

As Reddit encourages community participation, many questions are ``community seeking'' as opposed to \textit{information}-seeking. 
To identify information-seeking questions, we use \instructgpt\cite{ouyang2022training} to filter medical questions from non-medical questions (Prompt~\ref{prompt:med-v-non-med}) then manually vet the final set of 297 questions. 
We randomly sample 200 questions for our evaluation dataset and 50 questions for our development set, discarding the rest. 

Titles of Reddit posts are often a hook or a summary of the entire post. 
Using the 50 development questions, we use \instructgpt{} to minimally edit the titular question to include crucial details from the post description, providing a series of exemplars (Prompt~\ref{prompt:reddit-rewrite}).
These rewrites mainly include the age of a newborn or the stage of pregnancy from the description, but sometimes include small situational details that contextualize the question.
Two authors validate all rewrites, keeping the original title wherever both authors agree that the rewrite changed the communicative goal of the asker. 

\paragraph{Natural Questions.} Lastly, we include maternal and infant health questions from \abr{nq} to study pragmatic aspects of factoid-style questions.
We embed all questions in the train set of \abr{nq} using the \texttt{sentence-transformers}~\cite{reimers-2019-sentence-bert} implementation of \texttt{all-mpnet-base-v2}~\cite{DBLP:journals/corr/abs-2004-09297}, including unanswerable questions~\cite{asai-choi-2021-challenges}. 
We identify 2500 answerable questions and 2500 unanswerable questions as maternal health-related by identifying the top 100 nearest neighbors of 50 randomly sampled questions from the development sets of Reddit and \abr{rosie}.\footnote{We tried several different filtering heuristics, including keyword-based detection, but the nearest neighbors approach yielded the most topical questions.}
From this set, we randomly sample 100\footnote{\nq{} questions make up a smaller proportion of our evaluation dataset as we avoid diverting large amounts of annotation resources to factoid-style questions.} questions for our evaluation set and 50 for our development set.
Though obtained with a nearest neighbors approach, these questions greatly differ from those obtained from our previous sources, as they reflect the factoid \abr{qa}-oriented tasks and goals of the original dataset creators (Table~\ref{tab:dataset-sizes}).


\paragraph{Collecting Human Answers from Health Experts.} 
We recruit a team of twenty health experts using Upwork\footnote{\texttt{\url{https://www.upwork.com/}}} to annotate our data including obstetricians and gynecologists (OB/GYNs), nurses, lactation consultants, and public health experts, many of whom have experience with patients. 
In addition, many of these expert annotators are either currently pregnant or postpartum or have been in the past.
We ask a subset of six experts to write helpful and informative long-form answers to all 500 questions in our dataset (Figure~\ref{fig:annotation-instructions}, bottom panel).
While annotators write answers from scratch, they must provide supporting web documents from the same list of verified sources we use to build the corpus for \abr{rosie}.

\subsection{Identifying Assumptions and Implications}

Inferring \textit{possible} assumptions, implications, and asker beliefs from patient questions in our domain are challenging.
In the past, others have extracted assumptions using shallow signals from the surface form of a question~\cite{kim-etal-2021-linguist, parrish-etal-2021-nope}. 
While some assumptions or implications in our dataset can be inferred directly from the question expression, others require deeper domain or experiential knowledge (Table~\ref{table:dataset-examples}). 

Eliciting these assumptions and implications from non-linguists is challenging as existing linguistic frameworks (\S\ref{sec:pragmatic-primer}) are inaccessible or cumbersome for those unfamiliar with the theoretical concepts behind them. 
As such, we operationalize large-scale data collection by asking five annotators from a \textit{different} subset of our expert annotator pool to first write a list of subquestions that an answer to the original question would address (Figure~\ref{fig:annotation-instructions}, top panel). 
Doing so primes annotators to reason about the intent behind a question as well as the information needs of an asker.
Then, we ask them to write a set of sentences reflecting possible beliefs or assumptions that the patient may hold (or, alternatively, beliefs that any complete answer to the question must address).
We emphasize that the assumptions they write can be either medically or scientifically true or false.

Then, we \textit{consolidate} the set of subquestions and human-written assumptions and beliefs into a single set of assumptions and implications using \instructgpt (Prompt~\ref{prompt:question-consolidation}).

\subsection{Annotating Inference Veracity}

Lastly, we ask a new subset of eight expert annotators to annotate whether each assumption and implication in our dataset is medically or scientifically true, false, or subjective and provide a supporting web document from our list of verified sources along with a passage from the document (Figure~\ref{fig:annotation-instructions}, middle panel).

\paragraph{Validation.}
To verify that the assumptions and implications we extract are plausibly inferrable from the question, we recruit an additional pair of health experts, which we refer to as expert \textit{validators}, to rate inferences.\footnote{These expert validators were not a part of our dataset construction.}
We sample 100 assumptions and implications judged as false or subjective, and 100 true inferences and ask our expert validators to rate the plausibility of an inference on a 1--5 Likert scale based on how likely the question asker is to believe the assumption or implication. 
Henceforth, we refer to this sample of 200 inferences coming from 152 unique questions as \sample{}.
Both annotators judge the majority of our inferences as plausible, with 80\% and 95\% rated with a score of at least 3 (see Figure~\ref{fig:inference-validation} for the rating scale).
Spearman’s correlation between the two annotators is 0.69. See Appendix~\ref{appendix:validation-details} for more detail.








==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/sections/30-pragmatics-primer.tex <==
Assumptions and implications in our dataset map to two well-studied phenomena in linguistic pragmatics: presupposition and implicature~\cite{grice1975logic, stalnaker1977pragmatic}.
We begin with a short primer of both types of \textit{pragmatic inference} (\S~\ref{sec:pragmatic-primer}) and then discuss the implications of both types in a \abr{qa} setting (\S~\ref{sec:qa-implications}).

\subsection{Two Types of Pragmatic Inference: Presupposition and Implicature}
\label{sec:pragmatic-primer}

A sentence~\textit{S} is a \textit{pragmatic inference} of a
question~\textit{Q} if, depending on the \textit{context}
and \textit{conversational goals} of discourse
participants~\cite{jeretic-etal-2020-natural}, a human would believe that the asker of~$Q$ believes or
assumes~$S$ to be true.
Henceforth, we refer to the assumptions and implications that we collect in our dataset as \textit{pragmatic inferences}.
We review the two most relevant types of pragmatic inferences:
\textit{presupposition} and \textit{implicature}.

\paragraph{Presupposition.} Presuppositions are implicit assumptions in utterances taken for granted by
discourse participants~\cite{beaver1997presupposition}.
The question \textit{``What vitamins should I stop taking after
  becoming pregnant?''} presupposes \textit{``I was taking vitamins
  before becoming pregnant.''}
Presuppositions can often be detected solely 
by the presence of a lexical or syntactic
trigger~\cite{levinson1983pragmatics}.
In the example above, the word \textit{stop} presupposes that an
activity was already in motion.
We refer to these presuppositions as ``trigger-based''. 

As we observe during the collection of our dataset, domain or world knowledge is often needed to
capture presuppositions in real-world data that are not apparent from lexical or
syntactic cues~\cite{abusch2002lexical}.
For example, the question \textit{``Are multiple ultrasounds dangerous for my baby?''} does not directly result in non-trivial trigger-based presuppositions.
However, the asker of the question presupposes that the effects of an ultrasound are additive and hence asks about whether that additive effective is \textit{dangerous}.

\begin{figure*}[t!]
\centering
\includegraphics[scale=0.32]{figures/inference_type_dist.pdf}
\caption{Tree-map~\cite{shneiderman1992tree} visualizing the distribution of expert-annotated pragmatic inferences in \sample{} with their veracity, inference type, and whether or not they were addressed or not in the expert-written answer to the question from which they came from. When users make false or subjective inferences, they are more likely to do so as an implicature. Moreover,  when an inference is false, it is more likely to be naturally addressed in an answer by public health experts.}
\label{fig:inference-type-dist}
\end{figure*}


\paragraph{Implicature.} Implicature is a type of pragmatic inference that is
\textit{suggested} by an utterance as opposed to part of its literal
meaning~\cite{grice1975logic}.
Consider the question \textit{``Do most babies fit in newborn clothes?''}
While the speaker understands that newborn clothes fit \textit{some} babies,
their question implies that not all babies fit in newborn clothes.
As we discover, a significant portion of inferences in our dataset are
\textit{implied} from questions rather than presupposed, but detecting
and generating implicatures remain understudied in \abr{nlp}.

Some implicatures are related to lexical items or syntactic
structure of utterances. 
For example, the statement \textit{``These prenatal vitamins are in gumdrop form, \underline{but} are healthy''} implies that gumdrops are usually \emph{not} healthy.
Others are a function of a speaker's intent, beliefs, and other
contextual elements~\cite{zheng-etal-2021-grice}.
While they are a part of the content of an utterance, these implicatures are not \textit{at-issue} (e.g. the main point under discussion~\cite{potts2004logic, koev2018notions}) and are not encoded by the linguistic properties of
a sentence~\cite{ConversationalImplicature}.
Consider the question \textit{``How can you tell the difference between postpartum depression and exhaustion?''}. 
Reasoning about asker belief, we may conclude that they are implying that the two conditions should be treated differently, as one is more serious than the other.

\subsection{Presupposition and Implicature in \qa{}}
\label{sec:qa-implications}

In a natural setting, as we discover, humans embed both presuppositions and implicatures nearly equally in questions (\S\ref{sec:ask-and-answer}).
However, from a linguistic perspective, they represent different
levels of an asker's commitment to the propositional content of the
inference~\cite{peters2016speaker}.
Presuppositions are already a part of an asker's world model. 
In contrast, implicatures are \textit{likely} beliefs that may be negated in an asker's subsequent utterances.
Consider the question \textit{``Is it normal for my baby to move more than usual when closer to due date?''} with both the presupposition \textit{``There are factors that contribute to changes in fetal movement as the due date approaches''} and the implicature \textit{``It may not be necessary to be concerned if there is a significant increase in fetal movement close to the due date.''}
While both are false, the presupposition is stronger, and is clearly in need of addressing in a potential answer.
As illustrated, these distinct phenomena must be dealt with differently when answering a question.

\paragraph{Related Work.} Existing work in pragmatics in \qa{} focuses on open-domain question answering.
\citet{kim-etal-2021-linguist} present the first study of
presuppositions in Google search queries using the Natural Questions
(\abr{nq}) dataset~\cite{kwiatkowski-etal-2019-natural} that are
unanswerable due to false presuppositions.
However, their system only addresses trigger-based presuppositions, overlooking the type of deeper presuppositions present in our dataset derived from world or domain knowledge.
Other work has looked at Google queries with \textit{questionable} assumptions~\cite{Kim2022QA2QA} and false presuppositions in open-domain Reddit questions~\cite{Yu2022CREPEOQ}.
Computational studies of implicature have only focused on specific types, such
as scalar implicature (e.g., some $X$ $\rightarrow$ not all $X$)
\cite{schuster-etal-2020-harnessing, zheng-etal-2021-grice,
  kabbara-cheung-2022-investigating, jeretic-etal-2020-natural}.
As a result of the context induced by our domain, implicatures in our dataset extend beyond scalar implicature.


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/sections/40-ask-and-answer.tex <==
Before we investigate the behavior of \qa{} systems, we first study
how humans embed pragmatic inferences in their questions
(\S\ref{sec:pragmatic-inference-type}) as well as to what extent they
are \textit{naturally} addressed by human public health experts
(\S\ref{sec:de-novo-support}).

\subsection{Pragmatic Inference Type: Understanding Speaker Commitment}
\label{sec:pragmatic-inference-type}

When users ask questions, how strongly are they committed to the inferences that experts identify in their questions?
Presupposition is a phenomenon based on \textit{mutual} acknowledgment
of facts: when a human makes a presupposition, not only are they
presuming the content of the inference, they are also signaling the
belief that their \textit{interlocutor} (here, a \qa{} system) should
believe it too.

On the other hand, implicatures are a softer way for humans to express
uncertainty.
For example, \textit{``Which immunity injections can I skip for my baby?''} and \textit{``Is it sufficient if my baby takes most immunity injections''} have the same underlying inference (\textit{``It is okay to pick and choose vaccines''}), but is taken for granted in the first (presupposition), whereas loosely suggested in the second (implicature).
We want to distinguish inferences---separating implicatures from presuppositions---in our questions to better characterize \textit{so that we can prioritize addressing stronger false inferences.}

\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{figures/qa_pipeline.pdf}
\caption{Our baseline and pragmatic inference-augmented \abr{qa} pipelines. We experiment with retrieval, reranking, and reading stages and a variety of instruction-tuned and prompt-based models.}
\label{fig:model-pipeline}
\end{figure*}

\paragraph{Annotation Framework.}
A pair of authors independently annotate all inferences in \sample{}
as a presupposition or implicature by first determining whether it is a
proposition about the world that the asker believes to be true,
without which the question would not be felicitous (presupposition) or
whether it involves deriving asker belief through communicative
principles (implicature).
Between authors, Cohen's kappa is $\kappa=0.85$, indicating strong agreement. 
Author annotators adjudicated the final inference type (see Figure~\ref{fig:inference-type-dist} for overall distribution), but individual annotator labels and adjudication rationales are preserved as a part of our dataset.

\paragraph{Findings.}
Presuppositions and implicatures are balanced in \sample{}
(Figure~\ref{fig:inference-type-dist}), with a slight majority of
inferences as implicatures, indicating that many inferences that
health expert annotators identify are more subtle.
When an inference is true, it is almost equally likely to be a presupposition or an implicature. 
However, when users make false or subjective (veracity marked ``Unsure'') inferences, \textbf{they are more likely to do so via implicature} (Figure~\ref{fig:inference-type-dist}).
Past work has looked into generating and verifying
\textit{presuppositions} in open-domain \qa{}, but identifying and addressing \textit{implicatures} in an effort to make answers
information-complete remains heavily underexplored.
This finding highlights a key strength of our work: the ensuing context from our specific domain tests the usefulness of pragmatic inference in \abr{qa} by allowing us to extract a greater range of inferences.

In settings that lack such context (e.g. single-turn open-domain \abr{qa}), we are restricted to leveraging lexical or syntactic signals from the surface form of the question~\cite{kim-etal-2021-linguist} since reasoning about asker belief is not possible without other contextual signals.
For example, in the absence of additional context, the question \textit{``Should I push grandparents for flu shot and tdap?''}~may give rise to inferences involving the safety or effectiveness of these vaccines for the elderly.
However, upon learning that this was asked in a web forum by a postpartum mother, we may reason that she believes her infant may be at risk for contracting the flu or other diseases if their grandparents handle them unvaccinated.


\subsection{Addressing Inferences in Expert Answers}
\label{sec:de-novo-support}
When health experts are tasked with \textit{answering} questions, how likely are they to naturally address inferences that users implicitly make?
Studying whether or not answers \textit{naturally} address pragmatic inferences (\S~\ref{sec:de-novo-support}) gives us better insight into the types of inference health experts, and in turn models, should prioritize when answering questions.

\paragraph{Annotation.} We ask two annotators from our expert annotator pool to determine whether each inference in \sample{} is addressed, either implicitly or explicitly, by the human-written answer to its source question. 

\paragraph{Findings.} The majority of inferences in \sample{} are addressed by the human-written answer \textit{naturally} (Figure~\ref{fig:inference-type-dist}).
Importantly, \textbf{when an inference is false, it is more likely to be naturally addressed.}
Moreover, a significant number of \textit{true} inferences are also addressed by an answer, indicating that health experts not only aim to correct false or subject inferences but also prioritize completeness.
This key finding supports one of the main arguments of this work: \qa{} systems \textit{must} address pragmatic inferences in their answers, just as humans do.


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/sections/50-improve-qa.tex <==
Inducing pragmatic behavior in \qa{} systems is not straightforward.
Existing systems are not trained to proactively reason about asker beliefs, since many popular \qa{} datasets do not necessitate this type of behavior (e.g. factoid \qa{}).

We experiment with eliciting model answers that address the pragmatic needs of questions, such as refuting false inferences, using the pragmatic inferences in our dataset.
We inject inferences at each stage of the classic \qa{} pipeline: passage retrieval, reranking, and machine reading (\S\ref{sec:qa-system}) and evaluate outputs against expert-written answers with both automatic and human evaluation (\S\ref{sec:qa-eval}).

\subsection{Experimental Setup}
\label{sec:qa-system}

\paragraph{Corpus.} We use the corpus from \citet{mane2023practical} of 408,000 documents from verified web sources on maternal health and infant care and augment the corpus with the sources that our expert annotators found while both writing answers and determining the veracity of inferences.

\paragraph{Baseline Models.} As a baseline system, we use a retrieval, reranking, and reading-based \abr{qa} pipeline.
Contriever~\cite{izacard2022unsupervised}, an unsupervised dense passage retriever, identifies top relevant documents ($n=100$) in our corpus given a question.
Those documents are reranked using \abr{tart}-full~\cite{asai2022task}, a multi-task retrieval system with a cross-encoder architecture (Instruction~\ref{prompt:tart-baseline}). \abr{tart} is instruction-tuned, equipping it with the flexibility to redefine passage relevance for different tasks.
We feed the top five reranked documents to three different reader models: \abr{flan-t\small5-xxl}~\cite[11 billion parameters]{chung2022scaling}, an instruction-tuned, \textit{prompt}-based encoder-decoder model jointly trained on a multiple tasks with a standard answer extraction prompt from~\citet{naturalinstructions} (Instruction~\ref{prompt:flan-t5-reader}), \abr{mistral-\small7B}~\cite{jiang2023mistral} (an open source large language model, Prompt~\ref{prompt:mistral-gpt-reader}), and \instructgpt (Prompt~\ref{prompt:mistral-gpt-reader}).

\paragraph{Augmenting Systems with Pragmatic Inferences.} In addition to retrieving the top 100 passages using the question as input, we retrieve the top 100 passages for each pragmatic inference of the question ($i_1$...$i_k$) as well. 
Then, for each pragmatic inference $i$, we rerank the top 100 passages using a new inference-informed instruction (Instruction~\ref{prompt:tart-inference}) and select the top passage post-reranking.
We augment the top five reranked passages from the question with these $k$ top passages from each pragmatic inference to feed to each reader (Prompt~\ref{prompt:inference-augmented-reader}).
During reading, we prompt \abr{mistral-7B} and \instructgpt{} to address all $k$ assumptions when generating an answer.\footnote{We do not use \abr{flan-t5-xxl} here because it struggled with reading in the baseline setting.}
To keep the same \textit{number} of passages fed to readers in the baseline pipelines as in the inference-augmented pipeline, we add $k$ extra passages to the top five existing ones. 
This ensures that while the volume of information presented to machine readers is the same in both pipelines, the nature of the content differs, allowing us to measure the utility of inference augmentation during retrieval and reranking.
Figure~\ref{fig:model-pipeline} visualizes our baseline and inference-augmented \abr{qa} pipelines.

\input{tables/main-qa}

\subsection{Evaluation}
\label{sec:qa-eval}

We evaluate answers from seven pipeline variations against expert answers (Table~\ref{tab:main-qa-table}):
(1) The \textbf{No Reader} baselines consist of the top retrieved passage based on the input question (\abr{retrieve-only}) and the top reranked passage from the input question (\abr{rerank-only}),
(2) three \textbf{Baseline Readers} (\abr{baseline-flan-t5-xxl}, \abr{baseline-mistral-\small7B}, and \abr{baseline-gpt-\small3.5}), and
(3) two \textbf{Inference-Augmented} pipelines \abr{inference-mistral-\small7B}, and \abr{inference-gpt-\small3.5}). 

\paragraph{Automatic Evaluation Metrics.} Three automatic evaluation metrics measure the quality of generated answers: \abr{rouge}~\cite{lin-2004-rouge} (both F1 and recall),\abr{bleurt}~\cite{sellam-etal-2020-bleurt}, and \abr{QaFactEval}~\cite{fabbri-etal-2022-qafacteval}, a more recent QA evaluation metric originally designed to measure the faithfulness of summaries. 
\instructgpt{} scores the strongest according to \abr{QaFactEval}, our main evaluation metric because it---of the three metrics---most closely captures information content.
However, automatic evaluation of generated answers does \textit{not} capture several higher-level semantic and pragmatic aspects of the question.
Thus, we still need experts to validate the answers.

\paragraph{Human Judgments.}
We ask our expert \textit{validators} to score answers from the top-performing baseline and inference-augmented pipeline (\abr{baseline-gpt-\small3.5} and \abr{inference-gpt-\small3.5}, on \abr{QaFactEval} respectively).
For each of the 152 questions in \sample{}, expert validators score both model outputs simultaneously from 1--5 based on completeness (instructions in Figure~\ref{fig:annotation-instructions-qa-eval}). 
Answers typically received a score of 1 when they were off-topic and missing crucial information, a score of 2 when they were topical but still missing crucial information, 3 when containing all essential information to the question, 4 when most information was present for completeness, and a score of 5 when the answer was information complete.
Judging the information completeness of an answer is a subjective task, as reflected by the Spearman rank correlation between their annotations ($\rho=0.34$). 
While the mean score of inference-augmented examples is comparable to baseline answers ($4.43$ vs. $4.45$), annotators rated the inference-augmented answer as equivalent or better than its baseline counterpart in 75\% of questions in \sample{} (see Table~\ref{tab:generation-examples} for examples).


We further focus on annotator preferences on our original motivating population of questions---those with highly plausible, false assumptions. 
Both annotators rate inference-augmented answers higher than the default answers in the subset of questions with at least one \emph{highly plausible}, (plausibility=5) \emph{false} pragmatic inference (Table \ref{tab:highly-plausible-false}). 
We hypothesize that the similar ratings received by the two systems across \emph{all} questions is due to shortcomings in the instruction-following capabilities of LLMs. 
Forcing the reader model to address pragmatic inferences distracts it from answering the question more completely, and does not always result in more helpful answers when the pragmatic inferences are true.
These results illustrate the promise of inducing pragmatic behavior in \qa{} models and represent a lower bound of their performance, as none of the models we experiment with were trained to optimize for addressing assumptions in questions.


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/sections/60-generation.tex <==
While pragmatic inferences elicited from health experts are informed by their expertise, they are slow and costly to collect.
Our \qa{} experiments use \textit{human-written inferences} to
establish an upper bound of answer quality with existing models.
However, a fully automatic pragmatic \abr{qa} pipeline must first generate pragmatic inferences relevant to a question and \textit{then}
generate an answer that addresses the subset of false inferences.
As such, we experiment with generating pragmatic inferences with
\instructgpt\cite{ouyang2022training} to understand to what extent automating the process is feasible with existing prompting and in-context learning.

\paragraph{Experimental Setup.} We generate inferences with \instructgpt{} for all questions in \sample{} using seven in-context examples corresponding to 37 different pragmatic inferences, as more
in-context examples yields diminishing
returns~\cite{liu-etal-2022-makes}.
We select pragmatic inferences written by
multiple expert annotators from diverse user questions and
randomly shuffle them to prevent unwanted effects emerging from example order~\cite{si-relability-2022}, including exemplars from all three sources (\abr{rosie}, Reddit, and \nq{}) to capture distributional differences in their pragmatic inferences.
As humans naturally did, we let \instructgpt{} generate \textit{varied} numbers of inferences per
question.

\paragraph{Evaluation: Can \instructgpt generate human-like pragmatic inferences?}
For each inference in \sample{}, a pair of authors annotate whether or not each human-written assumption is semantically equivalent to at least one inference generated by \instructgpt (Prompt~\ref{prompt:inference-generation}) with a Cohen's kappa of $\kappa=0.88$.
Post-adjudication, 63\% of inferences were not present among model generations. 
When stratifying by inference type, 53\% of presuppositions and 71\% of implicatures were not present.
This illustrates that just as they are more difficult to detect, implicatures grounded in domain knowledge are more difficult for language models to generate.


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/sections/70-conclusion.tex <==
We show that it is possible to induce pragmatic behavior in \abr{qa} systems to correct latent false assumptions in the sensitive domain of
maternal and infant health.
Next-generation \abr{qa} systems deployed in real-world settings \textit{must} learn to address the pragmatics of user questions.
Though we have shown the viability of \textit{explicitly} inducing pragmatic behavior in models in this work, directions for future work include training retrievers to inherently search for evidence to address pragmatic inferences and readers to reason on top of such evidence to tactfully and effectively challenge user beliefs.


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/sections/acks.tex <==
We thank Philip Resnik, Sweta Agarwal, Sathvik Nair, and other members of the University of Maryland CLIP lab for their helpful feedback.
We also thank Ximena Marin Gutierrez, Marina Yue, Michelle Jasczynski, and Amara Channell Doig for their help in the development of \abr{rosie}.
We are grateful for our pool of expert annotators and for users of \abr{rosie} participating in our clinical trial.

The study reported in this paper was supported by research grants from the National Institute on Minority Health and Health Disparities (grant number R01MD016037) and by the National Library of Medicine (grant number R01LM012849). The content is solely the responsibility of the authors and does not necessarily represent the official views of the National Institutes of Health. The funders had no role in study design, data collection and analysis, decision to publish, or preparation of the paper.


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/sections/ethics.tex <==
\abr{nlp} systems are never a replacement for doctors or clinical expertise, especially in high-stakes settings. 
This work has grown out of collaboration with public health experts to help disseminate medically accurate but \textit{contextual} information to new or expectant mothers with limited access to healthcare.
Upon detection of false or potentially problematic assumptions, patients can then be referred to healthcare providers better able to provide information than current \abr{qa} systems.
All of our data was collected with \abr{irb} approval in consultation with public health professionals.  


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/sections/limitations.tex <==
\paragraph{Data are not multilingual.} 
Although our participants who provide questions come from diverse socioeconomic and racial backgrounds, all of the data we collect are in English. 
In addition, since we require participants to be located in the United States, the questions provided by participants are only reflective of the healthcare needs of English-speaking residents in the United States.

\paragraph{Choice of a single domain.}
While our approach can be generalized to any other domain, all of our data and experiments are confined to a single domain (maternal and infant health). 
We have not validated that our conclusions generalize beyond this particular important domain.
\paragraph{Pragmatics can be annotator-dependent.}
Finally, some degree of pragmatic inference is always dependent on the annotator, and we have not validated that this is consistent across different annotator backgrounds.


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/style/preamble.tex <==






\usepackage[a-1b]{pdfx}

\usepackage{framed}
\usepackage{mdwlist}
\usepackage{siunitx}
\usepackage{latexsym}
\usepackage{colortbl}
\usepackage{xcolor}
\usepackage{nicefrac}
\usepackage{booktabs}
\usepackage{fnpct}
\usepackage{amsfonts}
\usepackage[T1]{fontenc}
\usepackage{bold-extra}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{graphicx}
\usepackage{mathtools}
\usepackage{microtype}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{placeins}
\usepackage{xpatch}
\usepackage{latexsym,comment}
\usepackage[normalem]{ulem}

\newcommand{\breakalign}{\right. \nonumber \\ & \left. \hspace{2cm}}

\newcommand*{\missingreference}{{\Huge \colorbox{red}{?reference?}}}
\newcommand*{\missingcitation}{{\Huge \colorbox{red}{?citation?}}}

\makeatletter
\xpatchcmd{\@setref}{\bfseries}{\missingreference}{}{}
\def\@citex[#1]#2{\leavevmode
    \let\@citea\@empty
    \@cite{\@for\@citeb:=#2\do
        {\@citea\def\@citea{,\penalty\@m\ }%
            \edef\@citeb{\expandafter\@firstofone\@citeb\@empty}%
            \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}\fi
            \@ifundefined{b@\@citeb}{\hbox{\reset@font\missingcitation}%
                \G@refundefinedtrue
                \@latex@warning
                {Citation `\@citeb' on page \thepage \space undefined}}%
            {\@cite@ofmt{\csname b@\@citeb\endcsname}}}}{#1}}
\makeatother

\newcommand{\feat}[1]{{\small \texttt{#1}}}
\newcommand{\act}[1]{{\small \texttt{#1}}}
\newcommand{\ngram}[0]{$n$-gram}
\newcommand{\topic}[1]{\underline{#1}}
\newcommand{\gem}[1]{\mbox{\textsc{gem}}}
\newcommand{\abr}[1]{\textsc{#1}}
\newcommand{\camelabr}[2]{{\small #1}{\textsc{#2}}}
\newcommand{\abrcamel}[2]{{\textsc #1}{\small{#2}}}
\newcommand{\grammar}[1]{{\color{red} #1}}
\newcommand{\explain}[2]{\underbrace{#2}_{\mbox{\footnotesize{#1}}}}
\newcommand{\dir}[1]{\mbox{Dir}(#1)}
\newcommand{\bet}[1]{\mbox{Beta}(#1)}
\newcommand{\py}[1]{\mbox{\textsc{py}}(#1)}
\newcommand{\td}[2]{\mbox{\textsc{TreeDist}}_{#1} \left( #2 \right)}
\newcommand{\yield}[1]{\mbox{\textsc{Yield}} \left( #1 \right)}
\newcommand{\mult}[1]{\mbox{Mult}( #1)}
\newcommand{\wn}{\textsc{WordNet}}
\newcommand{\twentynews}{\textsc{20news}}
\newcommand{\g}{\, | \,}
\newcommand{\Gam}[1]{\Gamma \left( \textstyle #1 \right)}
\newcommand{\LG}[1]{\log \Gamma \left( \textstyle #1 \right)}
\newcommand{\Pois}[1]{\mbox{Poisson}(#1)}
\newcommand{\pcfg}[3]{#1_{#2 \rightarrow #3}}
\newcommand{\grule}[2]{#1 \rightarrow #2}
\newcommand{\kl}[2]{D_{\mbox{\textsc{KL}}} \left( #1 \,||\, #2 \right)}

\newcommand{\digambig}[1]{\Psi \left( #1 \right) }
\newcommand{\digam}[1]{\Psi \left( \textstyle #1 \right) }
\newcommand{\ddigam}[1]{\Psi' \left( \textstyle #1 \right) }


\renewenvironment{quote}
{\list{}{\rightmargin\leftmargin}%
    \item\relax\small\ignorespaces}
{\unskip\unskip\endlist}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\bmat}[1]{\text{\textbf{#1}}}
\newcommand{\bvec}[1]{\boldsymbol{#1}}

\newcommand{\emaillink}[1]{{\small \href{mailto://#1}{\texttt{#1}}}}
\newcommand{\smallemaillink}[2]{{\small \href{mailto://#2}{\texttt{#1}}}}

\newcommand{\ch}[1]{\begin{CJK*}{UTF8}{gbsn}#1\end{CJK*}}

\newcommand{\e}[2]{\mathbb{E}_{#1}\left[ #2 \right] }
\newcommand{\h}[2]{\mathbb{H}_{#1}\left[ #2 \right] }
\newcommand{\ind}[1]{\mathds{1}\left[ #1 \right] }
\newcommand{\ex}[1]{\mbox{exp}\left\{ #1\right\} }
\newcommand{\D}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\elbo}{\mathcal{L}}

\newcommand{\hidetext}[1]{}
\newcommand{\ignore}[1]{}

\ifcomment
    \newcommand{\pinaforecomment}[3]{\colorbox{#1}{\parbox{.8\linewidth}{#2: #3}}}

    \newcommand{\prtodo}[1]{\pinaforecomment{lightblue}{pr}{#1}}
    \newcommand{\prtodoi}[1]{\pinaforecomment{lightblue}{pr}{#1}}
\else
    \newcommand{\pinaforecomment}[3]{}
    \newcommand{\prtodo}[1]{}
    \newcommand{\prtodoi}[1]{}
\fi

\newcommand{\jbgcomment}[1]{\pinaforecomment{red}{JBG}{#1}}
\newcommand{\mjpcomment}[1]{\pinaforecomment{blue}{MJP}{#1}}
\newcommand{\czcomment}[1]{\pinaforecomment{orange}{chen}{#1}}
\newcommand{\clscomment}[1]{\pinaforecomment{blue}{CLS}{#1}}
\newcommand{\ffcomment}[1]{\pinaforecomment{red}{FF}{#1}}
\newcommand{\fpcomment}[1]{\pinaforecomment{green}{FP}{#1}}
\newcommand{\yhcomment}[1]{\pinaforecomment{green}{YH}{#1}}
\newcommand{\hhecomment}[1]{\pinaforecomment{blue}{HH}{#1}}
\newcommand{\tncomment}[1]{\pinaforecomment{blue}{TN}{#1}}
\newcommand{\mnicomment}[1]{\pinaforecomment{green}{Mohit}{#1}}
\newcommand{\prcomment}[1]{\pinaforecomment{lightblue}{Pedro}{#1}}
\newcommand{\fscomment}[1]{\pinaforecomment{orange}{Shi}{#1}}
\newcommand{\vmcomment}[1]{\pinaforecomment{yellow}{Varun}{#1}}
\newcommand{\rscomment}[1]{\pinaforecomment{yellow}{Richard}{#1}}
\newcommand{\jszcomment}[1]{\pinaforecomment{green}{JSG}{#1}}
\newcommand{\ascomment}[1]{\pinaforecomment{blue}{AS}{#1}}
\newcommand{\vecomment}[1]{\pinaforecomment{blue}{VE}{#1}}
\newcommand{\halcomment}[1]{\pinaforecomment{magenta!20}{Hal}{#1}}
\newcommand{\kgcomment}[1]{\pinaforecomment{blue}{Kim}{#1}}
\newcommand{\vancomment}[1]{\pinaforecomment{green}{VAN}{#1}}
\newcommand{\thangcomment}[1]{\pinaforecomment{green}{Thang}{#1}}
\newcommand{\alvincomment}[1]{\pinaforecomment{cyan}{Alvin}{#1}}
\newcommand{\reviewercomment}[1]{\pinaforecomment{blue}{Reviewer}{#1}}
\newcommand{\brscomment}[1]{\pinaforecomment{blue}{BRS}{#1}}
\newcommand{\psrcomment}[1]{\pinaforecomment{yellow}{PSR}{#1}}
\newcommand{\zkcomment}[1]{\pinaforecomment{cyan}{ZK}{#1}}
\newcommand{\swcomment}[1]{\pinaforecomment{yellow}{SW}{#1}}
\newcommand{\shaycomment}[1]{\pinaforecomment{yellow}{SBC}{#1}}
\newcommand{\jlundcomment}[1]{\pinaforecomment{cyan}{J}{#1}}
\newcommand{\kdscomment}[1]{\pinaforecomment{ceil}{KDS}{#1}}
\newcommand{\lkfcomment}[1]{\pinaforecomment{yellow}{LF}{#1}}
\newcommand{\yfcomment}[1]{\pinaforecomment{brown}{YF}{#1}}
\newcommand{\ewcomment}[1]{\pinaforecomment{lightblue}{Eric}{#1}}
\newcommand{\pgcomment}[1]{\pinaforecomment{lightblue}{Pranav}{#1}}
\newcommand{\dpcomment}[1]{\pinaforecomment{cyan}{Denis}{#1}}
\newcommand{\bencomment}[1]{\pinaforecomment{lightblue}{Ben}{#1}}
\newcommand{\mycomment}[1]{\pinaforecomment{pink}{Michelle}{#1}}
\newcommand{\nrcomment}[1]{\pinaforecomment{red}{Naveen}{#1}}
\newcommand{\ahcomment}[1]{\pinaforecomment{yellow}{Hoyle}{#1}}
\newcommand{\ahintext}[1]{{\small\textcolor{red}{[#1 -- \textsc{hoyle}]}}}
\newcommand{\mscomment}[1]{\pinaforecomment{lightblue}{Matt}{#1}}
\newcommand{\rrcomment}[1]{\pinaforecomment{lightblue}{RR}{#1}}
\newcommand{\nehacomment}[1]{\pinaforecomment{cyan}{Neha}{#1}}

\newcommand{\smalltt}[1]{ {\tt \small #1 }}
\newcommand{\smallurl}[1]{ \begin{tiny}\url{#1}\end{tiny}}
\newenvironment{compactenum}{ \begin{enumerate*} \small }{ \end{enumerate*} }

\definecolor{lightblue}{HTML}{3cc7ea}
\definecolor{CUgold}{HTML}{CFB87C}
\definecolor{grey}{rgb}{0.95,0.95,0.95}
\definecolor{ceil}{rgb}{0.57, 0.63, 0.81}
\definecolor{UMDred}{HTML}{ed1c24}
\definecolor{UMDyellow}{HTML}{ffc20e}


\newcommand{\qb}[0]{\abr{qb}}
\newcommand{\qa}[0]{\abr{qa}}
\newcommand{\odqa}[0]{\abr{odqa}}
\newcommand{\nlp}[0]{\abr{nlp}}
\newcommand{\dpr}[0]{\abr{dpr}}
\newcommand{\ml}[0]{\abr{ml}}
\newcommand{\triviaqa}{\camelabr{Trivia}{qa}}
\newcommand{\ambigqa}{\camelabr{Ambig}{qa}}
\newcommand{\searchqa}{\camelabr{Search}{qa}}
\newcommand{\wikiqa}{\camelabr{Wiki}{qa}}
\newcommand{\newsqa}{\camelabr{News}{qa}}
\newcommand{\trecqa}{\camelabr{Trec}{qa}}
\newcommand{\qblink}{\abrcamel{qb}{Link}}
\newcommand{\qanta}{\textsc{qanta}}
\newcommand{\muse}{\textsc{muse}}
\newcommand{\squad}{\textsc{sq}{\small u}\textsc{ad}}
\newcommand{\nq}[0]{\abr{nq}}
\newcommand{\conll}{\textsc{c}{\small o}\textsc{nll}}
\newcommand{\hotpot}{\abr{h}{\small otpot}\abr{qa}}
\newcommand{\fever}{\abr{fever}}
\newcommand{\quac}{\textsc{q}{\small u}\textsc{ac}}
\newcommand{\elmo}{\textsc{elm}{\small o}}
\newcommand{\fone}{$F_1$}
\newcommand{\jeopardy}{\textit{Jeopardy!\ }}

\newcommand{\glove}{\abr{gl}{\small o}\abr{ve}}
\newcommand{\openie}{\abr{o}{\small pen}\abr{ie}}
\newcommand{\bert}{\abr{bert}}
\newcommand{\drqa}{\abr{d}{\small r}\abr{qa}}
\newcommand{\docqa}{\abr{d}{\small oc}\abr{qa}}


\newcommand{\convo}[2]{
    \begingroup
    \addtolength\leftmargini{-0.2in}
    \begin{quote}
    \vspace{-0.5em}
    \small
        \textbf{Speaker A:} \textit{{#1}}
        \\
        \textbf{Speaker B:} \textit{{#2}}
    \vspace{-0.5em}
    \end{quote}
    \endgroup
}

\newenvironment{packed_enumerate}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}



==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/tables/annotation-examples.tex <==
\begin{table*}
\centering
\resizebox{2.08\columnwidth}{!}{
\begin{tabular}{p{0.18\linewidth}p{0.48\linewidth}p{0.6\linewidth}} 
\toprule
& \multicolumn{1}{c}{\textbf{Question}} & \multicolumn{1}{c}{\textbf{Expert-Annotated Pragmatic Inference \& Veracity}} \\ 
\midrule
\textbf{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\abr{rosie}\\(Maternal Health\\QA System) \end{tabular}}} & \texttt{Is it okay for my to color my hair after giving birth?}                & Hair dye chemicals can pass through breast milk from mother to child. (\falseunsure)\\
\arrayrulecolor[rgb]{0.753,0.753,0.753}\cline{2-3}
& \texttt{What is the advantage for not having an epidural during the labor?}    & Avoiding an epidural contributes to a more "natural" and unmedicated birthing experience. (\falseunsure)\\
\cline{2-3}
& \texttt{What cough medicine is appropriate for breastfeeding mothers?} & Some cough medicines can be secreted in breast milk. (\true)\\ 
\arrayrulecolor{black}\midrule
\multirow{3}{*}{\textbf{Reddit}}                                                             & \texttt{Is it safe to lay on my stomach at 28 weeks of pregnancy?} & Sleeping on the stomach while pregnant may have potential risks (\falseunsure) \\
\arrayrulecolor[rgb]{0.753,0.753,0.753}\cline{2-3}
& \texttt{Is it bad to use different bottles/nipples during feedings?} & Using different bottles or nipples for feeding may compromise the baby's latch. (\falseunsure) \\
\cline{2-3}
& \texttt{How can I increase the time between feedings for my 3-month-old baby?} & It may be possible to sleep through the night while still ensuring the baby is fed. (\true)\\ 
\arrayrulecolor{black}\midrule
\multirow{3}{*}{\textbf{Natural Questions}}  & \texttt{When does the fetus begin to develop memory?}  & Fetuses have the ability to form memories. (\true)  \\
\arrayrulecolor[rgb]{0.753,0.753,0.753}\cline{2-3}
& \texttt{What causes a rupture in the amniotic sac?} & There may be ways to prevent early amniotic sac rupture. (\falseunsure)\\
\cline{2-3}
& \texttt{When do the clinical manifestations of an ectopic pregnancy appear?}    & There may be clinical manifestations of an ectopic pregnancy that do not appear early on. (\true)\\
\arrayrulecolor{black}\bottomrule
\end{tabular}
}
\caption{Health experts identify pragmatic inferences from questions from three sources: Reddit, Natural Questions~\cite{kwiatkowski-etal-2019-natural}, and questions asked to our domain-specific \qa{} system, \abr{rosie}~\cite{mane2023practical}. They also determine the veracity of each inference and provide supporting evidence from a trusted web document.}
\label{table:dataset-examples}
\end{table*}


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/tables/dataset.tex <==
\begin{table}
\centering
\footnotesize
\setlength\tabcolsep{2pt}
\begin{tabular}{lccc} 
\toprule
                    & \begin{tabular}[c]{@{}c@{}}\textbf{Maternal Health}\\\textbf{QA}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Reddit}\\\textbf{}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Natural}\\\textbf{Questions}\end{tabular}  \\ 
\midrule
\textbf{\# questions}        & 200                                                                                  & 200             & 100                                                                           \\
\textbf{ans. length (\# sent)}    & 3.9                                                                                  & 6.6             & 5.6                                                                           \\
\textbf{\# inferences }      & 1161                                                                                 & 1114            & 452                                                                           \\
\>\>\>\% false/subjective & \textcolor[rgb]{0.125,0.129,0.141}{22.5}                                             & 30.8            & 20.1                                                                          \\
\>\>\>\% true             & 77.5                                                                                 & 69.2            & 79.9                                                                          \\
\bottomrule
\end{tabular}
\caption{Dataset statistics stratified by question source.}
\label{tab:dataset-sizes}
\end{table}


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/tables/generation-examples.tex <==
\begin{table*}[!ht]
\small
\centering
\resizebox{2.08\columnwidth}{!}{
    \begin{tabular}{p{0.15\linewidth}p{0.45\linewidth}p{0.45\linewidth}}
    \toprule
    \multicolumn{1}{c}{\colorbox{lightpurple}{\textcolor{darkpurple}{\textbf{Question ($Q$)}}}}
    & \multicolumn{1}{c}{\colorbox{lightteal}{\textcolor{teal}{\textbf{Default Answer} ($A_D$)}}} 
    & \multicolumn{1}{c}{\colorbox{lightteal}{\textcolor{teal}{\textbf{Pragmatic Inference-Augmented Answer} ($A_{IA}$)}}} \\ 
    \midrule
    When should I give my baby fever reducing meds after shots? &
    You should give your baby fever reducing medication after shots if they are experiencing discomfort or extreme discomfort due to the fever. However, it is important to note that in most cases, a child does not need to be medicated for a fever unless they are extremely uncomfortable. The most important thing to do when a child has a fever is to make sure they stay hydrated by drinking plenty of fluids. If you are unsure whether your child should receive medication to address the fever or other symptoms, it is recommended to consult with your child's healthcare provider. &
    \textbf{It is not recommended to give your baby fever reducing medication before or immediately after receiving shots. Studies have shown that giving medication prior to a vaccine visit may decrease the child's immune response to the vaccine. Fevers after vaccination are actually a sign that the immune system is responding to the vaccine.} If your baby develops a fever after receiving shots, it is generally not necessary to give them medication unless they are extremely uncomfortable. The most important thing to do when a child has a fever is to make sure they stay hydrated by drinking plenty of fluids. If you are unsure whether your baby should receive medication to address the fever or other symptoms, it is best to consult with your child's healthcare provider.
    \\
    \midrule
    How warm can my bath be while staying safe for my 4-month-old baby? &
    To ensure the safety of your 4-month-old baby during bath time, it is recommended to fill the basin with water that feels warm, but not hot, to the inside of your wrist or elbow. The water temperature should be comfortable for your baby and should not pose a risk of burns or scalds. It is important to check the water temperature before placing your baby in the bath to prevent any potential harm. &
    The safe temperature for a baby may be different from that for an adult. It is important to ensure that the bathwater is warm, but not hot, for a 4-month-old baby. According to the provided information, the water should feel warm to the inside of your wrist or elbow. It is recommended to fill the basin with 2 inches of water at this warm temperature. This is to prevent the baby from getting burned or scalded by hot water. \textbf{It is important to note that babies are not as adaptable as adults to temperature change, and they can lose heat rapidly. Therefore, it is crucial to maintain a safe and comfortable water temperature for the baby during bath time.} \\
    \toprule
    Can pregnancy tests be trusted? &
    According to pregnancy kit manufacturers, most at-home pregnancy tests are 98\% to 99\% accurate when used exactly as instructed. This means that positive results can generally be trusted. However, it is important to note that false negative results can occur if the test is taken too soon. Therefore, it is recommended to wait until a sufficient amount of time has passed since the possible conception before taking a pregnancy test to ensure more accurate results. &
    According to the information provided by pregnancy kit manufacturers, most at-home pregnancy tests are 98\% to 99\% accurate when used exactly as instructed. Positive results from these tests can be trusted. However, it is important to note that false negative results can occur if the test is taken too soon. \textbf{Blood tests, on the other hand, can detect pregnancy sooner and are the only tests that can show specific amounts of HCG in the body...} \\
    \bottomrule
    \end{tabular}
}
\caption{Outputs generated by a standard \abr{qa} system and a \abr{qa} systems informed by pragmatic inferences. Answers from the pragmatic system better explicate their underlying inferences.}
\label{tab:generation-examples}
\end{table*}


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/tables/high_plausibility.tex <==
\begin{table}
\centering
\small
\setlength\tabcolsep{2pt}
\begin{tabular}{lcc} 
\toprule
                    & \begin{tabular}[c]{@{}c@{}}\textbf{Mean Likert Score: }\\\textbf{Default Answer}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Inference-}\\\textbf{Augmented}\end{tabular}\\ 
\midrule
\textbf{Expert Annotator 1}        & 4.45   & 4.6  \\
\textbf{Expert Annotator 2}    & 4.37   & 4.45    \\
\bottomrule
\end{tabular}
\caption{Human preferences of answers on questions with at least one high-plausibility false assumption.}
\label{tab:highly-plausible-false}
\end{table}


==> nfqtfhhqgdfsmrxnncxmnjdqvfqbgtjp_arXiv/tables/main-qa.tex <==
\begin{table*}
\centering
\small
\setlength\tabcolsep{2.4pt}
\begin{tabular}{lcc|ccc|cc} 
\toprule
 & \multicolumn{2}{c|}{\textbf{No Reader}} & \multicolumn{3}{c|}{\textbf{Baseline Reader}}     & \multicolumn{2}{c}{\textbf{Inference-Augmented}}  \\ 
\midrule
 & \abr{Retrieve}~   & \abr{Rerank}                 & \abr{Flan-T5-XXL}  & \abr{Mistral-7B}   & \instructgpt      & \abr{Mistral-7B}   & \instructgpt                            \\ 
\midrule
\textbf{ROUGE-L (F1)}                                                                & $15.6_{(10.3)}$  & $17.5_{(10.3)}$    & $15.89_{(13.7)}$    & $17.4_{(5.1)}$   & $18.7_{(6.0)}$   & $16.2_{(4.8)}$   & $18.6_{(5.9)}$                         \\
\textbf{ROUGE-L (Recall)}                                                            & $23.0_{(15.7)}$  & $19.5_{(10.9)}$           & $36.9_{(21.9)}$   & $15.2_{(6.8)}$   & $17.4_{(8.1)}$   & $13.2_{(5.7)}$   & $16.6_{(7.6)}$                         \\
\textbf{BLEURT}                                                                      & -$0.72_{(0.34)}$ & -$0.61_{(0.29)}$          & -$0.79_{(0.45)}$ & -$0.38_{(0.22)}$ & -$0.37_{(0.22)}$ & -$0.36_{(0.21)}$ & -$0.38_{(0.22)}$                       \\
\textbf{\abr{QaFactEval}}                                                     &    $0.69_{(1.05)}$     &    $0.76_{(0.80)}$        &       $1.16_{(1.5)}$      &        $1.02_{(0.65)}$      &     $1.15_{(0.73)}$         &      $0.96_{(0.62)}$        &           $1.17_{(0.75)}$                         \\
\textbf{Human (/5)} & -            & -                        & -            & -            &     $4.43$         & -            &      $4.45$                            \\
\bottomrule
\end{tabular}
\caption{Mean and standard deviations of automatic (\abr{rouge}, \abr{bleurt}, \abr{QaFactEval}) and human evaluation metrics per question. We report results for the top retrieved passage and the top reranked passage, and two modes with and without access to human-written assumptions. Inference-augmented models perform competitively with baselines, indicating the promise of inducing pragmatic behavior in \qa{} models to mitigate harm.}
\label{tab:main-qa-table}
\end{table*}


==> scripts/git-latexdiff <==
#! /bin/bash

# Main author: Matthieu Moy <Matthieu.Moy@imag.fr> (2012 - 2016)
# (See the Git history for other contributors)
#
# Copying and distribution of this file, with or without modification,
# are permitted in any medium without royalty provided the copyright
# notice and this notice are preserved.  This file is offered as-is,
# without any warranty.
#
# git-latexdiff is a wrapper around latexdiff
# (http://www.ctan.org/pkg/latexdiff) that allows using it to diff two
# revisions of a LaTeX file.
#
# The script internally checks out the full tree for the specified
# revisions, calls latexpand to flatten the document and then calls
# latexdiff, hence this works if the document is split into multiple
# .tex files.
#
# Try "git latexdiff -h" for more information.
#
# To install, just copy git-latexdiff in your $PATH.

# Missing features (patches welcome ;-):
# - diff the index
# - hardlink temporary checkouts as much as possible

# Alternatives:
#
# There is another script doing essentially the same here:
# https://github.com/cawka/latexdiff/blob/master/latexdiff-git
# My experience is that latexdiff-git is more buggy than
# git-latexdiff, but they probably just don't have the same bugs ;-)
#
# There are a bunch of other alternatives cited here:
#
#   http://tex.stackexchange.com/questions/1325/using-latexdiff-with-git
#
# Ideally, these scripts should be merged.

set -o errexit
set -o noclobber

# Some versions of git set $GIT_WORK_TREE when ran through an alias.
# This wouldn't work with git-latexdiff which plays with different
# work trees.
unset GIT_DIR
unset GIT_WORK_TREE

# (Comment and 'unset' line borrowed from Git's source code)
# Having this variable in your environment would break scripts because
# you would cause "cd" to be taken to unexpected places.  If you
# like CDPATH, define it for your interactive shell sessions without
# exporting it.
# But we protect ourselves from such a user mistake nevertheless.
unset CDPATH

# @GIT_LATEXDIFF_VERSION@ is substituted by the install script here,
# but not within git_latexdiff_compute_version().
git_latexdiff_version='@GIT_LATEXDIFF_VERSION@'

git_latexdiff_compute_version () {
    if [ "$git_latexdiff_version" = '@GIT_LATEXDIFF''_VERSION@' ]; then
	(cd "$(dirname "$0")" && git describe --tags HEAD 2>/dev/null || echo 'Unknown version')
    else
	echo "$git_latexdiff_version"
    fi
}

usage () {
    cat << EOF
Usage: $(basename "$0") [options] OLD [NEW]
       $(basename "$0") [options] OLD --
       $(basename "$0") [options] -- OLD
Call latexdiff on two Git revisions of a file.

OLD and NEW are Git revision identifiers. NEW defaults to HEAD.
If "--" is used for NEW, then diff against the working directory.

Options:
    --help                this help message
    --main <file.tex>     name of the main LaTeX file
    --no-view             don't display the resulting PDF file
    --latex               run latex instead of pdflatex
    --bibtex, -b          run bibtex as well as latex
                             (pdflatex,bibtex,pdflatex,pdflatex)
    --biber               run BibLaTex-Biber as well as latex
                             (pdflatex,bibtex,pdflatex,pdflatex)
    --view                view the resulting PDF file
                            (default if -o is not used)
    --pdf-viewer <cmd>    use <cmd> to view the PDF file (default: \$PDFVIEWER)
    --no-cleanup          don't cleanup temp dir after running
    --no-flatten          don't call latexpand to flatten the document
    --cleanup MODE        Cleanup temporary files according to MODE:

                           - keeppdf (default): keep only the
                                  generated PDF file

                           - none: keep all temporary files
                                  (may eat your diskspace)

                           - all: erase all generated files.
                                  Problematic with --view when the
                                  viewer is e.g. evince, and doesn't
                                  like when the file being viewed is
                                  deleted.

    --latexmk             use latexmk
    --latexopt            pass additional options to latex (e.g. -shell-escape)
    -o <file>, --output <file>
                          copy resulting PDF into <file> (usually ending with .pdf)
                          Implies "--cleanup all"
    --tmpdirprefix        where temporary directory will be created (default: /tmp)
    --verbose, -v         give more verbose output
    --quiet               redirect output from subprocesses to log files
    --prepare <cmd>       run <cmd> before latexdiff (e.g. run make to generate
                             included files)
    --ln-untracked        symlink uncommited files from the working directory
    --version             show git-latexdiff version.
    --subtree             checkout the tree at and below the main file
                             (enabled by default, disable with --whole-tree)
    --whole-tree          checkout the whole tree (contrast with --subtree)
    --ignore-latex-errors keep on going even if latex gives errors, so long as
                          a PDF file is produced
    --ignore-makefile     ignore the Makefile, build as though it doesn't exist
    -*                    other options are passed directly to latexdiff
    --bbl                 shortcut to flatten a bbl file of the same name as the project
    --latexpand           pass options to latexpand (should be last option specified)
    --latexdiff-flatten   use --flatten from latexdiff instead of latexpand
EOF
}

die () {
    echo "fatal: $*"
    exit 1
}

verbose () {
    if test "$verbose" = 1 ; then
	printf "%s ..." "$@"
    fi
}

verbose_progress () {
    if test "$verbose" = 1 ; then
	printf "."
    fi
}

verbose_done () {
    if test "$verbose" = 1 ; then
	echo " ${1:-done}."
    fi
}

verbose_say () {
    if test "$verbose" = 1 ; then
	printf "%s\n" "$@"
    fi
}

old=
new=
main=
view=maybe
cleanup=keeppdf
verbose=0
bibtex=0
biber=0
output=
initial_dir=$PWD
initial_repo=$(git rev-parse --show-toplevel)
tmpdir_prefix="/tmp"
prepare_cmd=
flatten=1
subtree=1
uselatexmk=
latexopt=
ln_untracked=0
quiet=0
ignorelatexerrors=0
latexdiffopt=()
latexpand=()
bbl=0
latexdiff_flatten=0
latex=0


while test $# -ne 0; do
    case "$1" in
        "--help"|"-h")
            usage
            exit 0
            ;;
	"--main")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    main=$1
	    ;;
	"--no-view")
	    view=0
	    ;;
	"--view")
	    view=1
	    ;;
	"--pdf-viewer")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    PDFVIEWER="$1"
	    ;;
	"--no-cleanup")
	    cleanup=none
	    ;;
	"--ignore-latex-errors")
	    ignorelatexerrors=1
	    ;;
        "--cleanup")
            shift
            case "$1" in
                "none"|"all"|"keeppdf")
                    cleanup="$1"
                    ;;
                *)
                    echo "Bad argument --cleanup $1"
                    usage
                    exit 1
                    ;;
            esac
            ;;
	"--no-flatten")
            flatten=0
            ;;
	"--ignore-makefile")
	    ignoremake=1
	    ;;
	"-o"|"--output")
	    test $# -gt 1 && shift || die "missing argument for $1"
	    output=$1
	    cleanup=all
	    ;;
	"-b"|"--bibtex")
	    bibtex=1
	    ;;
	"--latex")
	    latex=1
	    ;;
	"--biber")
	    biber=1
	    ;;
	"--verbose"|"-v")
	    verbose=1
	    ;;
        "--quiet")
	    quiet=1
	    ;;
	"--version")
	    git_latexdiff_compute_version
            exit 0
	    ;;
	"--subtree")
	    subtree=1
	    ;;
	"--whole-tree")
	    subtree=0
	    ;;
	"--prepare")
	    shift
	    prepare_cmd="$1"
	    ;;
        "--latexmk")
            uselatexmk=1
            ;;
	"--latexpand")
	    shift
	    latexpand=$1
	    ;;
	"--bbl")
	    bbl=1
	    ;;
	"--latexdiff-flatten")
	    latexdiff_flatten=1
            flatten=0
	    ;;
	"--latexopt")
	    shift
	    latexopt=$1
	    ;;
        "--ln-untracked")
            ln_untracked=1
            ;;
        "--no-ln-untracked")
            ln_untracked=0
            ;;
        "--tmpdirprefix")
	    shift
	    tmpdir_prefix="$1"
	    ;;
        -*)
            if test "$1" = "--" ; then
                if test -z "$new" ; then
                    new=$1
                else
                    echo "Bad argument $1"
                    usage
                    exit 1
                fi
            else
                latexdiffopt+=("$1")
            fi
            ;;
        *)
	    if test -z "$1" ; then
		echo "Empty string not allowed as argument"
		usage
		exit 1
	    elif test -z "$old" ; then
		old=$1
	    elif test -z "$new" ; then
		new=$1
	    else
		echo "Bad argument $1"
		usage
		exit 1
	    fi
            ;;
    esac
    shift
done

if test -z "$new" ; then
    new=HEAD
fi
if test "$new" = "--"; then
    ln_untracked=1
fi

if test -z "$old" ; then
    echo "fatal: Please, provide at least one revision to diff with."
    usage
    exit 1
fi

if test -z "$PDFVIEWER" ; then
    verbose "Auto-detecting PDF viewer"
    candidates="xdg-open evince okular xpdf acroread"
    if test "$(uname)" = Darwin ; then
        # open exists on GNU/Linux, but does not open PDFs
	candidates="open $candidates"
    fi

    for command in $candidates; do
	if command -v "$command" >/dev/null 2>&1; then
	    PDFVIEWER="$command"
	    break
	else
	    verbose_progress
	fi
    done
    verbose_done "$PDFVIEWER"
fi

case "$view" in
    maybe|1)
	if test -z "$PDFVIEWER" ; then
	    echo "warning: could not find a PDF viewer on your system."
	    echo "warning: Please set \$PDFVIEWER or use --pdf-viewer CMD."
	    PDFVIEWER=false
	fi
	;;
esac

if test $flatten = 1 &&
    ! command -v latexpand 2>/dev/null; then
    echo "Warning: latexpand not found. Falling back to latexdiff --flatten."
    latexdiff_flatten=1
    flatten=0
fi

if test $latex = 1; then
    LATEX_EXEC=latex
else
    LATEX_EXEC=pdflatex
fi    

## end option parsing ##

check_knitr () {
    if test -z "$prepare_cmd"; then
	prepare_cmd="Rscript -e \"library(knitr); knit('$main')\""
    fi
    main="${main%\.*}.tex"
}

log_cmd () {
    log=$1
    shift
    if [ "$quiet" = 1 ]; then
	"$@" >$log 2>&1
    else
	"$@"
    fi
}

# main is relative to initial_dir (if returned)
if test -z "$main" ; then
    printf "%s" "No --main provided, trying to guess ... "
    main=$(git grep -l '^[ \t]*\\documentclass')
    # May return multiple results, but if so the result won't be a file.
    if test -r "$main" ; then
	echo "Using $main as the main file."
    else
	if test -z "$main" ; then
	    echo "No candidate for main file."
	else
	    echo "Multiple candidates for main file:"
	    printf "%s\n" "$main" | sed 's/^/\t/'
	fi
	die "Please, provide a main file with --main FILE.tex."
    fi
fi

ext=${main##*\.}
case "$ext" in
    Rnw) check_knitr ;;
    Rtex) check_knitr ;;
    *) ;;
esac

if test ! -r "$main" ; then
    die "Cannot read $main."
fi

verbose "Creating temporary directories"

git_prefix=$(git rev-parse --show-prefix)
git_dir="$(git rev-parse --git-dir)" || die "Not a git repository?"
cd "$(git rev-parse --show-cdup)" || die "Can't cd back to repository root"
git_dir=$(cd "$git_dir"; pwd)

# make main relative to git root directory
if test -n "$git_prefix" ; then
    main=$git_prefix$main
fi
mainbase=$(basename "$main" .tex)
maindir=$(dirname "$main")

tmpdir=$tmpdir_prefix/git-latexdiff.$$
mkdir "$tmpdir" || die "Cannot create temporary directory."

cd "$tmpdir" || die "Cannot cd to $tmpdir"

mkdir old new || die "Cannot create old and new directories."

verbose_done
verbose_say "Temporary directories: $tmpdir/old and $tmpdir/new"
verbose "Checking out old and new version"

cd old || die "Cannot cd to old/"
if test "$ln_untracked" = 1; then
    (
       mkdir -p "$maindir" && cd "$maindir" && ln -s "$initial_repo"/"$maindir"/* .
    )
fi

if test "$subtree" = 1; then
    checkoutroot=$git_prefix
else
    checkoutroot="."
fi

# Checkout a subtree, without touching the index ("git checkout" would)
(cd "$git_dir" && git archive --format=tar "$old" "$checkoutroot") | tar -xf -
verbose_progress
cd ../new || die "Cannot cd to new/"
if test "$ln_untracked" = 1; then
    (
       mkdir -p "$maindir" && cd "$maindir" && ln -s "$initial_repo"/"$maindir"/* .
    )
fi
if test "$new" != "--"; then
    # if new == "--" then diff working dir (already there thanks to ln
    # -s above).
    (cd "$git_dir" && git archive --format=tar "$new" "$checkoutroot") | tar -xf -
fi
verbose_progress
cd ..

verbose_done

for dir in old new
do
    verbose "Running preparation command $prepare_cmd in $dir/$git_prefix"
    ( cd "$dir/$git_prefix/" && log_cmd prepare.log eval "$prepare_cmd" )
    if test ! -f "$dir/$main"; then
	die "$prepare_cmd did not produce $dir/$main."
    fi
    verbose_done
done

# Option to use latexdiff --flatten instead of latexpand
if test "$latexdiff_flatten" = 1; then
    latexdiffopt+=("--flatten")
fi

# Shortcut to include bbl
if test "$bbl" = 1; then
    bblexpand=("--expand-bbl" "$mainbase.bbl")
else
    bblexpand=()
fi

# Create flattened documents and keep for debugging
if test "$flatten" = 1; then
    if [ "$bbl" = 1 ]; then
	if [ ! -f "old/$maindir$mainbase.bbl" ]; then
	    verbose "Attempting to regenerate missing old/$maindir$mainbase.bbl"
	    oldPWD=$PWD
	    cd old/"$maindir"
	    log_cmd pdflatex0.log pdflatex $latexopt "$mainbase" || compile_error=1
	    log_cmd bibtex0.log bibtex "$mainbase" || compile_error=1
	    cd "$oldPWD"
	    if [ "$compile_error" = 1 ]; then
		die "Failed to regenerate .bbl for old version"
	    fi
	fi
	if [ ! -f "new/$maindir$mainbase.bbl" ]; then
	    verbose "Attempting to regenerate missing new/$maindir$mainbase.bbl"
	    oldPWD=$PWD
	    cd new/"$maindir"
	    log_cmd pdflatex0.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
	    log_cmd bibtex0.log bibtex "$mainbase" || compile_error=1
	    cd "$oldPWD"
	    if [ "$compile_error" = 1 ]; then
		die "Failed to regenerate .bbl for new version"
	    fi
	fi
    fi
    verbose "Running latexpand"
    (
	cd old/"$maindir" &&
	latexpand "$mainbase".tex "${latexpand[@]}" "${bblexpand[@]}"
    ) > old-"$mainbase"-fl.tex \
	|| die "latexpand failed for old version"
    (
	cd new/"$maindir" &&
	latexpand "$mainbase".tex "${latexpand[@]}" "${bblexpand[@]}"
    ) > new-"$mainbase"-fl.tex \
	|| die "latexpand failed for new version"
    verbose_done

    verbose "Running latexdiff ${latexdiffopt[*]} old-${mainbase}-fl.tex new-${mainbase}-fl.tex > ./diff.tex"
    latexdiff "${latexdiffopt[@]}" old-"$mainbase"-fl.tex new-"$mainbase"-fl.tex > diff.tex \
	|| die "latexdiff failed"
    verbose_done

    verbose "mv ./diff.tex new/$main"
    mv -f new-"$mainbase"-fl.tex new-"$mainbase"-fl.tex.orig
    mv -f diff.tex new/"$main"
    verbose_done
else
    verbose "Running latexdiff ${latexdiffopt[*]} old/$main new/$main > ./diff.tex"
    latexdiff "${latexdiffopt[@]}" old/"$main" new/"$main" > diff.tex \
	|| die "latexdiff failed"
    verbose_done

    verbose "mv ./diff.tex new/$main"
    mv -f new/"$main" new/"$main.orig"
    mv -f diff.tex new/"$main"
    verbose_done
fi

verbose "Compiling result"

compile_error=0
cd new/"$maindir" || die "Can't cd to new/$maindir"
if test -f Makefile && test "$ignoremake" != 1 ; then
    log_cmd make.log make || compile_error=1
elif test "$uselatexmk" = 1; then
    log_cmd latexmk.log latexmk -f -pdf -silent "$mainbase" || compile_error=1
else
    if [ "$ignorelatexerrors" = 1 ]; then
	latexopt="$latexopt -interaction=batchmode"
    elif [ "$quiet" = 1 ]; then
	latexopt="$latexopt -interaction=nonstopmode"
    else
	latexopt="$latexopt -interaction=errorstopmode"
    fi
    log_cmd pdflatex1.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
    if test "$bibtex" = 1 ; then
	log_cmd bibtex.log bibtex "$mainbase" || compile_error=1
    fi
    if test "$biber" = 1 ; then
	log_cmd biber.log biber "$mainbase" || compile_error=1
    fi
    log_cmd pdflatex2.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
    log_cmd pdflatex3.log $LATEX_EXEC $latexopt "$mainbase" || compile_error=1
fi

verbose_done

if [ "$compile_error" = 1 ] && [ "$ignorelatexerrors" = 1 ]; then
    echo "LaTeX errors were found - but attempting to carry on."
    compile_error=0
fi

if test $latex = 1; then
    dvips "$mainbase".dvi
    ps2pdf "$mainbase".ps
fi

pdffile="$mainbase".pdf
if test ! -r "$pdffile" ; then
    echo "No PDF file generated."
    compile_error=1
fi

if test ! -s "$pdffile" ; then
    echo "PDF file generated is empty."
    compile_error=1
fi

if test "$compile_error" = "1" ; then
    echo "Error during compilation. Please examine and cleanup if needed:"
    echo "Directory: $tmpdir/new/$maindir"
    echo "     File: $mainbase.tex"
    # Don't clean up to let the user diagnose.
    exit 1
fi

if test -n "$output" ; then
    abs_pdffile="$PWD/$pdffile"
    (cd "$initial_dir" && mv "$abs_pdffile" "$output")
    echo "Output written on $output"
elif [ -f "$pdffile" ]; then
    new_pdffile="$tmpdir"/"$pdffile"
    mv "$pdffile" "$new_pdffile"
    pdffile="$new_pdffile"
fi


if test "$view" = 1  || test "$view" = maybe  && test -z "$output" ; then
    "$PDFVIEWER" "$pdffile"
fi

case "$cleanup" in
    "all")
	verbose "Cleaning-up result"
	cd ..
	cd ..
	rm -fr "$tmpdir"
	verbose_done
	;;
    "keeppdf")
	verbose "Cleaning-up all but pdf (kept in $pdffile)"
	rm -fr "$tmpdir"/old "$tmpdir"/new
	verbose_done
	;;
    "none")
	verbose_say "Generated files kept in $tmpdir/"
	;;
esac


==> scripts/style-check/bad-words <==
utilize              % phrase "use" http://www.bartleby.com/64/C003/0294.html
utilizes             % phrase "uses" http://www.bartleby.com/64/C003/0294.html
utilized             % phrase "used" http://www.bartleby.com/64/C003/0294.html
utilizing            % phrase "using" http://www.bartleby.com/64/C003/0294.html
leverage             % phrase "use"
abstraction          % phrase this is often used poorly?
fashion              % phrase hrm.
[dw]on't             % spelling do not or will not.
behavioral           % spelling I'm convinced we don't use this word properly.
we'll                % spelling we will
we've                % spelling we have
[^r][^c][^h] impact  % phrase "consequences", "effect", "result", though nsf likes "research impact"
tackle               % phrase "tackle" (a problem) is wimpy for "solve" or a tired metaphor for "address a challenge".
thusly               % phrase "thus" or "this way" or "like this" http://www.bartleby.com/64/C003/0282.html
transpire            % phrase "happen" 
so-called            % phrase can be abused; it's negative.
necessitate          % phrase require.
necessitated         % phrase required.
necessitates         % phrase requires.
loosing              % spelling you almost certainly mean "losing".  use "loosening" otherwise.
aforementioned       % phrase too pretentious.
important to         % phrase "valued by"?
notion               % phrase avoid this weak phrase. (thanks brian bershad!)
achieve(s)?\s        % phrase models don't achieve anything, only use for humans
reasonably           % phrase hedging


==> scripts/style-check/common-typos <==
a the                % phrase double article
 pt                  % syntax ? I guess avoid straggling pt's that escape tex?
[ ],                 % syntax whitespace before comma seems wrong.
Figure Figure        % phrase pizza pizza.
[ ]-[ ]              % syntax a hyphen surrounded by space should probably be an emdash '---'
[0-9]-[0-9]          % syntax use an endash '--' for ranges
[0-9]ms              % syntax put a space between the number and the unit.
[^egs]\. [a-z]       % syntax a period usually ends a sentence, and sentences should start with a capital; doesn't apply for i.e.,
\.  [a-z]            % syntax a period usually ends a sentence, and sentences should start with a capital; "i.e." should have a comma following.
[a-z]\.\.            % syntax double period is rarely right, use \ldots for ellipsis
[^\\]"               % syntax use fancy quotes
\beg\.               % syntax should be e.g. as in "examples given"
from to\b            % phrase haven't used this properly.
help help            % phrase double word, that probably means the author paniced
of of                % phrase apparent double word.
the affect           % phrase should probably be 'the effect'
the the              % phrase apparent double word.
there too few        % phrase there are too few?
was not was          % phrase pretty much a joke if this gets matched.
we we                % phrase it would be oi oi in french, I guess.
with on              % phrase probably wrong.
with with            % phrase apparent double word.
[\n ]--[\n ]         % syntax that's an en-dash, you want an em-dash: "---"
my my                % phrase unlikely that's what you want, at least without a comma. (doesn't work across newlines)
>From                % syntax be careful when you email .tex files.  I've seen this slip through into submissions.
e\.t\.c\.            % syntax it's et cetera; use etc.
such as like         % phrase pick one
<<<<<<< .            % syntax CVS conflict!
=======              % syntax CVS conflict!
>>>>>>> [0-9]        % syntax CVS conflict!
e\.g\.[\n ]          % syntax should be followed with a comma, as e.g. can be read as "for example" (thanks JZ!)
i\.e\.[\n ]          % syntax should be followed with a comma, as i.e. can be read as "that is" (thanks JZ!)
[ ]\.[\n ]           % syntax stray period?
further more         % phrase one word: furthermore
safe guard           % phrase one word: safeguard
that be              % phrase mistake.
can not              % phrase cannot
only only            % phrase double word
is is                % phrase double word.
they shows           % phrase argh, mistake.
less that than       % phrase typo damage
from from            % phrase double word score
in in                % phrase "in" (common mistake)
not not              % phrase argh.
it it                % phrase argh.
to illicit           % phrase "to elicit" -- illicit is always an adjective.
c\.f\.               % phrase actually, it's cf., and you'd like cf.\ (backslash space)
this lead to         % phrase "led to" if past tense, "leads to" if present.
on on                % phrase double word.
has is               % phrase choose
description their    % phrase saw this, clearly wrong.
including:  % syntax I prefer no colon after including, which already says a list is coming.
[a-z]\([A-Z]  % syntax put a space before parens, even when introducing acronyms.
without and without % phrase saw this.
can be result       % phrase saw this typo.



==> scripts/style-check/foolish-phrases <==
(quite|more|very|most) unique    % phrase unique is.
(quite|more|very|most) abstract  % phrase abstract is.
tangible view                    % phrase mix that metaphor some more.
for e\.g\.                       % phrase e.g. includes "for".
begs the question                % phrase unless you're very clever: "raises the question": http://alt-usage-english.org/excerpts/fxbegthe.html
high rate of speed               % phrase local news-speak.
especially necessary             % phrase 'especially important', necessary may be an absolute like unique.
how will it effect % phrase you likely meant "affect"
how it will effect % phrase you likely meant "affect"
insure proper performance % phrase "ensure"
especially true                  % phrase 'especially important', true may be an absolute like unique.
to affect change                 % phrase "effect" change;  I read this on a poster.
higher results                   % phrase maybe higher performance or higher values.
is more general then the         % phrase probably "than"
upper bounding                   % phrase "limiting" or "setting an upper bound on"
in principal                     % phrase likely, "in principle"
literally like                   % phrase literally means no simile.  
design principal  % phrase likely, "design principle" 
different from 	    	   	 % phrase unlike

==> scripts/style-check/latex-checking <==
\{\\em [^\}]*[^\}\/]\}[:]    % syntax use \emph{} or explicit italic correction {\em foo\/}
\{\\em [^\}]*[:\.,]\}        % syntax punctuation at the edges of italic text is not italicized
[A-Z]{2,10}\.[ ]*[\n ][ ]*[A-Z]  % syntax intersentence spacing should be used if a sentence ends with an acronym: "FOO\\@."
\\etal[^{]                   % syntax it's good practice to use \etal{} to avoid bad spacing
\\caption\[[^\]]*[^\.]\]     % syntax short caption should end with a period.
\\caption\[.*CCDF.*\]        % syntax short caption should not include graph type.
\\caption\[.*CDF.*\]         % syntax short caption should not include graph type.
\\caption\[.{0,25}\]         % syntax short caption should not be too short.
th century                   % syntax use textsuperscript
[ ]---[ ]                    % syntax the em-dash should be right up against the words.
[ \n]---[ \n]                % syntax the em-dash should be right up against the words.
^---[ \n]                    % syntax the em-dash should be right up against the words.
[ \n]---$                    % syntax the em-dash should be right up against the words.
[ \n]--[ \n]                 % syntax the en-dash should be between numbers.
^--[ \n]                     % syntax the en-dash should be between numbers.
[ \n]--$                     % syntax the en-dash should be rbetween numbers.
,[~ ]\\etal                  % syntax no comma before etal (unless Smith, Martinez, \etal)
\\etal\{\}'s                 % syntax eew.
\\(sub)?section\{[A-Z][^}]*[ ][a-z]{5,40}[^}]*\} % syntax subsection headers should be initial capped.
\\(sub)?section\{[A-Z][^}]*[^:][ ]{1,}(With|A|An|Is|And|For|To|The)[ ][^}]*\} % syntax some words needn't be capitalized
[ ]\\footnote                % syntax no space before footnote.
\\footnote\{.*\}.            % syntax footnotes after punctuation
,,                           % syntax double comma is unlikely to be intentional.
cf\.[^\\]                    % phrase cf. should get an escaped space "\ "
et al\.[^\\]                    % phrase et al. should get an escaped space "\ "
[<>]  % syntax a less than or greater than outside math mode shows other characters.
in (section|table|figure) \\ref % phrase should have ~ before ref
section~\\ref % capitalize capitalize section when saying Section 6.
table~\\ref % capitalize capitalize section when saying Table 6.
figure~\\ref % capitalize capitalize section when saying Figure 6.
\\(sub)?section\{Intro\} % syntax spell it out.
,''                          % syntax punctuation outside quotes
\.\.\.                       % syntax use \dots

==> scripts/style-check/my-rules <==
#  such may be abused to blacklist certain words even spelled correctly.
# capitalize is case sensitive, and also bracketed by non-word.
# phrase and spelling are case insensitive, but bracketed by non-word characters.
# syntax is case sensitive but not bracketed by non-word; probably best if used with regexes.
\bet al\.[^}]        % syntax use the \etal{} command instead. (or write one to italicize)
\bet\. al\.          % syntax use the \etal{} command, "et" needs no dot (et alii). (or write one to italicize)
\bc\.f\.\b             % syntax should be cf. for "confer" (latin for compare)
\b$i\)[^$]              % syntax leave the paren in math mode -- should be $i)$
\b$ii\)[^$]             % syntax leave the paren in math mode -- should be $ii)$
\b$iii\)[^$]            % syntax leave the paren in math mode -- should be $iii)$
\b$iv\)[^$]             % syntax leave the paren in math mode -- should be $iv)$
\b$v\)[^$]              % syntax leave the paren in math mode -- should be $v)$
\ban [b-df-gj-np-tv-z] % syntax probably meant to use "a" instead of "an", though there are exceptions.
\ban [B-DF-GJ-NP-TV-Z][^A-Z/] % syntax probably meant to use "a" instead of "an", though there are exceptions (like acronyms).
\b[Aa] [aeiouAEIOU](?!se|ni|A|ur|RL|ti|ne|DP) % syntax probably meant to use "an" instead of "a", though there are exceptions. (user, useful, AA, unified, uniform, unique, Europe, one, UDP; n/a doesn't work, so use {n/a})
This allows           % phrase tie more explicitly: This (x) allows...
we find               % phrase omit "we find"
we found              % phrase omit "we found"
try and               % phrase "try to", though if you're using try as a noun in a compound sentence, this rule is wrong.
impact of             % phrase not a useful metaphor; try evaluation, success, effect, value.
including [^\.]*etc\. % syntax "including" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
includes [^\.]*etc\.  % syntax "includes" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
and etc\.             % phrase come on. learn some latin.
AT&T                  % syntax you poor thing, this won't compile.
doesn't               % phrase be formal.
be occur              % phrase what happens when I'm indecisive about what follows "can"
up until              % phrase "until"
one or more           % phrase probably redundant -- nonzero is probably implied.
is comprise(d|s) of   % phrase you probably mean "is composed of" because "comprises" is more a synonym for "contains" 
will be significantly different % phrase "will differ significantly" for active voice
More importantly,     % phrase probably means the order is wrong: put important stuff first.
todo                  % ignoredcommand
texttt                  % ignoredcommand
jbgcomment              % ignoredcommand
lkfcomment              % ignoredcommand
due to space constraints % phrase don't whine.
this paper % phrase can be ambiguous if talking about someone else's paper whether you mean the one youre writing or the one you're talking about..
the above             % phrase horrible phrase that must be expunged.  you might use "these" instead, but best to make the sentence stand alone.
referred to above     % phrase "these".
(all|the|of) [0-9][ ] %  phrase use words for numbers in phrases.
clearly shows         % phrase "clearly" is usually much.
grows larger          % phrase is "grows smaller" possible?  grows.
guarantee as much as possible % phrase then not really a guarantee "provide"
affects negatively   % phrase "hurts" or "harms"
rely upon % phrase rely on is good enough
relies upon % phrase relies on is good enough
record route packets? % phrase hyphenate record-route packets
record-route; % phrase leave record route alone if not modifying something else
we accomplish this  % phrase verbose way to get active voice.
refers to the % phrase you're being wimpy in the definition.  use "is"
\\emph\{[a-zA-Z ]*\} refers to % syntax you're being wimpy in the definition.
loss off % phrase loss of?
this could % phrase this "what" could
with that has % phrase probably just one
simply % phrase probably isn't.
to get to % phrase "to reach"?
latency benefit % phrase reduction
latency improvement % phrase reduction
shed insight % phrase 'shed light' would seem the metaphor.
increasingly more % phrase redundant
I\.e\. % syntax starting a sentence with i.e. is just ugly.
E\.g\. % syntax starting a sentence with e.g. is just ugly.
in the large % phrase if large is a noun, bad.  if it's an adjective, fine.
encapsulates with % phrase seen it, don't know what it means.
when working with % phrase just say "with"
it is true that	  % phrase usually can delete
LDA % phrase convention put in small caps
(F|f)indings (show|indicate|suggest)	% phrase delete or make more specific

==> scripts/style-check/networking-research <==
IPs                  % phrase should be IP addresses
[Rr]ate-limits       % spelling "rate limits" has no hyphen, only "rate-limited"
best effort          % phrase hyphenate best-effort service.
deliver route        % phrase jargon redundancy
euclidean % capitalize Euclidean.
interdomain          % spelling inter-domain
internet             % capitalize unless talking about an internet other than the Internet
intradomain          % spelling intra-domain
log-normal           % spelling lognormal is one word.
pareto               % capitalize
ttl                  % capitalize
weibull              % capitalize proper name.
PoP                  % syntax I think POP looks less annoying.
PoPs                 % syntax I think POP looks less annoying.
http[ ]              % capitalize capitalize HTTP.
linux                % capitalize capitalize Linux
Internet[^\.]*Internet % syntax avoid Internet twice in the same sentence?
zipf                 % capitalize capitalize the guy's name.


==> scripts/style-check/passive-voice <==
it is possible to                   % phrase passive voice, try: "can"
are identified by                   % phrase passive
is shown                            % phrase passive.
is not included in                  % phrase maybe this is passive
there (are|is) [^\.:;]* (that|in)   % phrase maybe this is passive
can be evaluated                    % phrase avoid passive: I evaluated
can be observed                     % phrase avoid passive: are visible
# is needed                         % phrase passive voice
is used to                          % phrase go active voice, or subsititute "helps"
(are|were) needed[^\?]              % phrase passive voice
(is|are) presented in               % phrase "appears in", or reword to avoid passive voice
it is possible that                 % phrase "may"
(is|are) (depicted|illustrated|sketched) in  % phrase thats passive voice
(is|are) shown in                   % phrase "shows"
as can be seen in                   % phrase X shows that Y.
there needs to be                   % phrase passive voice in a bad way.
was designed                        % phrase passive voce.
it may be                           % phrase passive "it"
it is important that                % phrase passive; replace with X is important because Y.


==> scripts/style-check/verbose-phrases <==
a large number of                   % phrase you mean "many"
a substantial number of             % phrase how substantial?  most?  or just enough that can't be ignored?
an insufficient number of           % phrase "too few"
a significant number of             % phrase one is significant.   consider "prohibitive" if the number is sufficient to be problematic.
a number of                         % phrase getting the verb agreement for this useless phrase is tricky.
a number of different               % phrase use "different" (should have a high score)
a small number of                   % phrase you mean "few"
a low number of                   % phrase you mean "few"
a relatively low number of                   % phrase you mean "few"
actually                            % spelling probably doesn't add
to an extent                        % phrase you can probably remove
and instead                         % phrase replace with but?
be done                             % phrase if "X of Y can be done", try "Y can be Xed"; it's already passive voice.
combining multiple                  % phrase as opposed to "combining one?"
aggregating multiple                % phrase "aggregating"
do this                             % phrase probably verbose if you use a pronoun for what you're doing
exists[ ]                           % phrase probably no better than "is", but end of sentence may be unavoidable?
if it is to                         % phrase should be "to" (usually followed by "be X")
if they are to                      % phrase should be "to" (usually followed by "be X")
in general                          % phrase unless matched with "in specific," this is usually useless; perhaps "overall"
in order to                         % phrase remove "in order" and get "to"
in the past                         % phrase past tense is likely enough.
in the way of                       % phrase should be "as"
counting the number of              % phrase counting.  dude.
is permitted to                     % phrase "may"
largely opaque                      % phrase largely does not modify opaque
makes a new                         % phrase should be "creates"
may not chose                       % phrase "may not" is future tense; "chose" is past.
one should note                     % phrase just write it.
note that                           % phrase is the rest of the paper less notable?
Note, that                          % syntax not only should you not "note that", no comma after note.
we note                             % phrase is the rest of the paper less notable?
note however that                   % phrase is the rest of the paper less notable?
it is important to note             % phrase is the rest of the paper less notable?
really                              % phrase probably doesn't add; if you think it does, use "r{}eally" -- don't change to 'in fact'
in fact				    % phrase cut
rigorously                          % spelling probably doesn't add, and I rarely do anything with rigor
the way in which                    % phrase should be "how" or ""
the manner in which                 % phrase should be "how" or ""
value stems                         % phrase value is derived or offered, I think.
time at which                       % phrase very likely "when"
place at which                      % phrase very likely "where"
at the time                         % phrase very likely "when"
reduced number of                   % phrase very likely "fewer" or maybe maybe "less"
is present in                       % phrase present is probably redudant, try "is in"
they all                            % phrase maybe "all xs" would be better.
easy to do                          % phrase "feasible" or "practical" might be better.
is going to                         % phrase "will".
are going to                        % phrase "will".
getting                             % phrase probably "receiving" or "querying"
those are                           % phrase see if "those X are" is clearer?
design is motivated                 % phrase "inspired by" is probably better than "motivated" for design
locations throughout the world      % phrase drop "throughout the world"
e.g., as opposed to                 % phrase if you're giving examples, you're not talking about what isn't.  drop "e.g."
in addition, we also                % phrase remove either "also" or "in addition"
other related issues                % phrase probably remove "other"
the aforementioned                  % phrase "these xs" or "this x" would be less snooty
center around                       % phrase (cook) a center is a point: "center on" is okay.
could care less                     % phrase (cook) 'really? how much less could you care?' (should be couldn't)
grouped together                    % phrase redundant.  "grouped" alone should suffice.
put together                        % phrase long: "construct" "build" or "assemble"
consistent with each other          % phrase redundant.  "consistent" suffices.
be accomplished with                % phrase try "requires" "uses" "needs"?
the lack of knowledge of            % phrase would "X is unknown" work better?
gets to know                        % phrase you mean "learns"
trying to look like                 % phrase you mean "acting", "emulating", or "mimicing"
has got to be                       % phrase "must be"
got                                 % phrase try "became" "received" ?
gotten                              % phrase try "helped" ?
live in a vacuum                    % phrase a tired metaphor that makes me want to vomit.
positive impact                     % phrase try "benefit"
negative impact                     % phrase try "harm" or "consequences"
adverse impact                      % phrase try "harm" or "consequences"
adversely impacting                 % phrase try "harming" or "hurting"
discuss the issues of               % phrase could probably drop "the issues of" unless there's a list
the presence of                     % phrase not far from 'is', 'has', etc.
does not allow                      % phrase consider "forbids" or "prohibits"
and/or                              % phrase just say or.
there is the potential to           % phrase just say may.
there is the possibility that       % phrase just say might.
can be achieved                     % phrase maybe not so good?
find out                            % phrase perhaps determine?
in the absence of                   % phrase perhaps without?
in the presence of                  % phrase perhaps with?
set up                              % phrase perhaps create, configure, or initialize
in the face of                      % phrase can be overused.  try despite?
several times (at|of)               % phrase discouraged by Kurt.
a large degree of                   % phrase ick.
we start by first                   % phrase redundant. ("first, we" or "we start by").
in general, they are usually        % phrase redundant.
refers to the notion                % phrase define your term precisely if possible.
a significant amount of             % phrase probably just "significant"
real practical                      % phrase as opposed to imaginary practical?
people that are                     % phrase use people who are?
additional detail that we add       % phrase as opposed to additional detail that we subtract?
in some cases and not in others     % phrase "in some cases"
it is known that                    % phrase just say it.
caused due to                       % phrase "caused by"
a result of the fact that           % phrase "caused by"
results (indicate|show|suggest)     % phrase drop
research (indicates|show|suggest)   % phrase drop
can be attributed to the fact that  % phrase "is because"
a large set of                      % phrase probably don't care that it is a set.
a small set of                      % phrase probably don't care that it is a set: use 'a few'
provides a look at                  % phrase (timid) probably mean "shows".
in most cases                       % phrase "usually"
continue into the forseeable future % phrase "continue".
for the forseeable future           % phrase drop.
fail to successfully                % phrase "fail to" is sufficient.
Clearly,                            % syntax starting a sentence with clearly confuses me.
in different continents             % phrase ON different continents, IN different countries
(we|to) handle                      % phrase use a more specific verb like address, treat, solve
handling                            % phrase use a more specific verb like addressing, treating, solving, mitigating (unless handling errors or exceptions)
For the purposes of                 % phrase "For"
We observe that                     % phrase drop.
some degree of                      % phrase "some"
in the problem of                   % phrase (contributed by rap)
conclude several things             % phrase make (draw) several conclusions
extra bonus                         % phrase "bonus"
added bonus                         % phrase "bonus"
it is important to emphasize that   % phrase use diction to emphasize.
it is possible that                 % phrase "x may y"
caused due to                       % phrase "caused by"
recent work by                      % phrase could maybe be dropped, as the cite will include the date.
identify the location of            % phrase "find"
that go across                      % phrase "that cross"
ideally, we would like              % phrase "we would like"
enabling the ability to             % phrase "supporting" or "allowing" or "permitting"
absolutely essential                % phrase essential is.
we essentially do                   % phrase essentially is a poor adverb.  "The essence of our algorithm is a..."
Essentially,                        % phrase maybe "In essence," but could also be removed.
In this section (we|I)              % phrase "In this section, we", or "In this section, I"
essentially all                     % phrase "most"
past experience                     % phrase "experience" http://www.cmu.edu/styleguide/trickywords.html
particulary difficult primarily     % phrase simplify
intuition about why                 % phrase "intuition as to why"
Recall from above                   % phrase "recall"
Further, (I|we) will also           % phrase drop further or also
respectively                        % phrase unneeded.
in terms of                         % phrase don't need this.
the extent to which                 % phrase "how much"
make sure                           % phrase "ensure"
make up                             % phrase "constitute" "compose"
make use of                         % phrase "use"
make a decision                     % phrase "decide"
make a guess                        % phrase "guess"
since that time                     % phrase "since then"
choices to make                     % phrase "choices"
certain limitations                 % phrase what does 'certain' add to limitations?
will [a-z]* in the future           % phrase "will"
business entities                   % phrase "businesses"
rely primarily on                   % phrase "primarily" weakens "rely".  perhaps just "use" would be simpler.
has the potential to                % phrase can
have not yet developed              % phrase "have yet to develop"
to be effective,                    % phrase probably redundant.
provide information about           % phrase "tell how" "reveal" "expose" "disclose"
are different,                      % phrase "differ"
have already been                   % phrase "have been"? "were"?
as appropriate                      % phrase not needed?
only rarely                         % phrase "rarely" is probably enough.
is effective at                     % phrase "can"
foremost among them is              % phrase "foremost is" would be shorter.
those that have no                  % phrase those without
that have no                        % phrase "without"?
a variety of diverse                % phrase redundant
be highly valuable in               % phrase simplify.
the overall goal                    % phrase 'the goal'
sometimes an? [a-z]+ will           % phrase an x may
this is perhaps because             % phrase this may be because
adding an additional                % phrase redundant
IP protocol                         % phrase redundant
works well                          % phrase be more specific.
something                           % phrase could eliminate.
to keep from                        % phrase "to avoid"
[\.,] since (!then)                 % phrase probably you mean "because" unless you're talking about time. -- "has since" is okay.
performance characteristics         % phrase rare that characteristics adds.
takes into account                  % phrase considers
specify particular                  % phrase if specifying, particular should be redundant.
prototype implementation            % phrase "implementation" is redundant.
given a particular                  % phrase "given a" is probably enough
described in detail (in|below)      % phrase use "detailed"
relatively more                     % phrase more is already relative.
focus primarily on                  % phrase bad metaphor: subject of focus is singular.
primary focus                       % phrase bad metaphor: subject of focus is singular.
relatively more                     % phrase more is already relative.
gives [a-z]+ [a-z]+ information about % phrase use "tells" x
gives [a-z]+ information about      % phrase use "tells" x
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
have an effect on                   % phrase "affect"
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
we can see                          % phrase "we can see" isn't formal enough.
still remain                        % phrase "remain".
change over time                    % phrase "change"
turn into                           % phrase "become"
looking back in retrospect          % phrase pick.
ensures that there will be no       % phrase "prevents"
does have                           % phrase "has"
first step toward this              % phrase "toward this" can probably be dropped.
can potentially be                  % phrase "might be", or just "can be"
obviates the need for               % phrase just obviates x, not obviates the need for x.
it is indeed                        % phrase "it is", though still passive.
planning in advance                 % phrase when else might you plan?
a lot of                            % phrase "many"
keep in mind                        % phrase "consider" (or drop)
it is clear that                    % phrase if clear, you don't have to say it.
especially true                     % phrase true is an absolute, can't be especially true.
making it increasingly difficult    % phrase preventing, discouraging, impeding, blocking, slowing...
is potentially                      % phrase "may be"
have been [a-z]* in the past        % phrase 'in the past' is redundant with tense.
amount of time  % phrase "duration"
should ideally % phrase "should"
are of great benefit to % phrase "help" or "aid"
are of benefit to % phrase "help" or "aid" or "promote"
important here % phrase consider "relevant"
while at the same time % phrase "while" is enough.
are able to % phrase can
subvert the proper operation of % phrase subvert
speed slow % phrase speed is probably redundant.
of size no smaller than % phrase "of size" is probably redundant
of size no larger than % phrase "of size" is probably redundant
of size smaller than % phrase "of size" is probably redundant
of size larger than % phrase "of size" is probably redundant
might potentially % phrase "might"
in the context of % phrase "in" avoid, if possible.
increase the amount of % phrase probably just increase.
show the difference between % phrase compare
in addition, we also % phrase pick.
overhead efficiency % phrase huh?
have an effect on % phrase "affect"
have a signficant effect on %  phrase "affect"
we find % phrase can usually be removed
this suggests % phrase remove or make more precise
effective for providing	   	 % phrase remove
we performed a                   % phrase just use the verb directly
we perform a                     % phrase just use the verb directly
were able to                     % phrase could
are able to                      % phrase can


==> tables/de_novo_support.tex <==
\begin{table}
\centering
\small
\begin{tabular}{lcc|c} 
\toprule
             & \textbf{Addressed} & \textbf{Not Addressed} & \textbf{Total}  \\ 
\midrule
\addlinespace[0.5pt]
\textbf{True}         & 33.5      & 16.5          & 50.0   \\
\textbf{False/Unsure} & 39.0      & 11.0          & 50.0   \\ 
\midrule
\textbf{Total}        & 72.5      & 27.5          & 100    \\
\addlinespace[-0.5pt]
\bottomrule
\end{tabular}
\caption{Distribution of human answers addressing inferences in \sample{} stratified by veracity. Majority of inferences in our dataset are addressed naturally by health expert annotators, especially when they are false.}

\label{tab:de-novo-support}
\end{table}


==> tables/head-to-head.tex <==
\begin{table}
\centering
\small
\setlength\tabcolsep{2pt}
\begin{tabular}{lcccc} 
\toprule
                    & \begin{tabular}[c]{@{}c@{}}\textbf{Mean Likert Score: }\\\textbf{Default Answer}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Inference-}\\\textbf{Augmented}\end{tabular}\\ &  \begin{tabular}[c]{@{}c@{}}\textbf{Inference-}\\\textbf{Augmented}\end{tabular} \ & \begin{tabular}[c]{@{}c@{}}\textbf{Inference-}\\\textbf{Augmented}\end{tabular}
\midrule
\textbf{Expert Annotator 1}        & 4.45   & 4.6  & 0 & 0 \\
\textbf{Expert Annotator 2}    & 4.37   & 4.45  & 0 & 0  \\
\bottomrule
\end{tabular}
\caption{Human preferences of answers on questions with at least one high-plausibility false assumption.}
\label{tab:highly-plausible-false}
\end{table}

==> tables/inference-type-veracity.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{
    \begin{tabular}{lccc} 
    \toprule
    \textbf{Pragmatic Inference Type} & \textbf{True} & \textbf{False} & \textbf{Unsure} \\ 
    \midrule
    Trigger Presupposition (\tp)  & \textbf{47.2} & 21.5 & 36.5 \\
    Non-Trigger Presupposition (\ntp) & 21.3 & 8.9 & 9.6 \\
    Conventional Implicature (\cni) & 2.3 & 2.5 & 0.0 \\
    Conversational Implicature (\cri) & 29.1 & \textbf{67.1} & \textbf{53.8} \\ 
    \midrule
    All & 61.2 & 22.4 & 16.4 \\
    \bottomrule
    \end{tabular}
}
\caption{Pragmatic inference veracity stratified by linguistic type. Veracity columns each sum to 1. The majority of \textit{false} inferences are conversational implicatures that are highly context-sensitive.}
\label{tab:veracity}
\end{table}

==> tables/inference_type.tex <==
\begin{table}
\centering
\small
\begin{tabular}{lcc|c} 
\toprule
               & \textbf{True} & \textbf{False/Unsure} & \textbf{Total}  \\ 
\midrule
\addlinespace[0.5pt] % Add extra space between rows

\textbf{Presupposition} & 25.5 & 20.0         & 45.5   \\
\textbf{Implicature}    & 24.5 & 30.0         & 54.5   \\ 
\midrule
\textbf{Total}          & 50.0 & 50.0         & 100    \\
\addlinespace[-0.5pt]
\bottomrule
\end{tabular}
\caption{Distribution of veracity and inference type in \sample{}. When users make false or subjective assumptions, they are more likely to do so via implicature.}
\label{tab:ask-inference-type}
\end{table}

==> tables/more-examples.tex <==
\begin{table*}[pt!]
\centering
\resizebox{2.00\columnwidth}{!}{
\begin{tabular}{lll} 
\toprule
\textbf{Original Question} & \textbf{Annotator-Edited Question} & \textbf{Pragmatic Inferences} \\ 
\hline
support your baby's head and neck? & How do I safely support my newborn's head and neck? & 1.~Babies' heads and necks are weak. \\ 
\hline
what music will my baby like? & What kind of music should I play my baby in the womb? & \begin{tabular}[c]{@{}l@{}}1. Babies can hear in the womb.\\2. Playing music is good for babies.\\3. Babies can differentiate music from other sound.\end{tabular} \\ 
\hline
can i have one cigarette a day without harming my baby? & Not Edited & \begin{tabular}[c]{@{}l@{}}1. Moderate smoking could minimize risks for baby\\2. Smoking more than one cigarette can hurt the baby.\end{tabular} \\ 
\hline
get a jump start on baby proofing? & What can I do to baby proof my home before the birth?\textcolor[rgb]{0.094,0.565,1}{}\textcolor[rgb]{0.094,0.565,1}{} & 1. Babyproofing can occur before birth. \\ 
\hline
what will do if baby got fever & What should I do if my baby has a fever?\textcolor[rgb]{0.094,0.565,1}{}\textcolor[rgb]{0.094,0.565,1}{} & \begin{tabular}[c]{@{}l@{}}1. Babies get fevers.\\\textcolor[rgb]{0.094,0.565,1}{}\textcolor[rgb]{0.094,0.565,1}{}2. There are ways to treat fevers.\textcolor[rgb]{0.094,0.565,1}{}\textcolor[rgb]{0.094,0.565,1}{}\\3. Fevers could have broader health effects.\textcolor[rgb]{0.094,0.565,1}{}\textcolor[rgb]{0.094,0.565,1}{}\\4.There is a normal temperature range for infants.\end{tabular} \\
\bottomrule
\end{tabular}
}
\caption{Examples of original user questions, annotators' edits to the original question, and their extracted pragmatic inferences.}
\label{tab:more-examples}
\end{table*}
